Peak Estimation of Time Delay Systems using Occupation Measures

This work proposes a method to compute the maximum value obtained by a state function along trajectories of a Delay Differential Equation (DDE). An example of this task is finding the maximum number of infected people in an epidemic model with a nonzero incubation period. The variables of this peak estimation problem include the stopping time and the original history (restricted to a class of admissible histories). The original nonconvex DDE peak estimation problem is approximated by an infinite-dimensional Linear Program (LP) in occupation measures, inspired by existing measure-based methods in peak estimation and optimal control. This LP is approximated from above by a sequence of Semidefinite Programs (SDPs) through the moment-Sum of Squares (SOS) hierarchy. Effectiveness of this scheme in providing peak estimates for DDEs is demonstrated with provided examples

==> sections/acknowledgements.tex <==
\section*{Acknowledgements}
J. Miller and M. Sznaier were partially supported by NSF grants  CNS--1646121, ECCS--1808381 and CNS--2038493, AFOSR grant FA9550-19-1-0005, and ONR grant N00014-21-1-2431.  
This material is based upon research supported by the Chateaubriand Fellowship of the Office for Science \& Technology of the Embassy of France in the United States.

The work of  M. Korda and V. Magron was partly supported by the European Union's Horizon 2020 research and innovation programme under the Marie Sklodowska-Curie Actions, grant agreement 813211 (POEMA). The work of M. Korda was also partly supported by the Czech Science Foundation (GACR) under contract No. 20-11626Y and by the AI Interdisciplinary Institute (ANITI) funding, through the French "Investing for the Future PIA3" program under the Grant  agreement ANR-19-PI3A-0004.



The authors would additionally like to thank Didier Henrion, Alexandre Seuret, and the BrainPOP group at LAAS-CNRS for their comments and support.

==> sections/conclusion.tex <==
\section{Conclusion}
% \urg{Unite this with the rest of the paper}
\label{sec:conclusion}

This paper presented a formulation of 
\ac{MV}-solutions for free-terminal-time \acp{DDE} with multiple histories (Definition \ref{defn:mv_solution}). These \ac{MV}-solutions are formed by the conjunction of Validity, Liouville and Consistency constraints.
These \ac{MV}-solutions may be used to provide upper bounds on peak estimation problems over \acp{DDE} by Program \eqref{eq:peak_delay_meas}.

% constructed from measures may be used to characterize the behavior of \ac{DDE} trajectories.  Peak Estimation problems for \acp{DDE} may be upper bounded by optimizing over a set of free-terminal time \ac{MV}-solutions.
% \ac{MV}-solutions of a \ac{DDE} given a single history $x_h$ are unique for fixed and free terminal time problems (where a distribution of stopping times are given for the free-time case). These \ac{MV}-solutions may be used to bound trajectory analysis problems such as peak estimation and reachable set estimation.
% \ac{MV}-solutions of \acp{DDE} will be used in subsequent chapters to formulate optimal control, peak estimation, and reachable set estimation problems. 
% One vital area for future work is determining under what conditions does it occur that each weak solution is supported on the graph of \ac{DDE} trajectories \cite{ambrosio2003lecture}. Such a statement would impose that there is no relaxation gap between the trajectory and measure programs, and therefore that the sequence of \ac{LMI} solutions will converge to the true optimum as the degree $d \rightarrow \infty$. 

A vital area for future work is determining the conditions under which $P^* = p^*$ between \eqref{eq:peak_delay_traj} and \eqref{eq:peak_delay_meas}.
Other areas for future work include applying \ac{MV}-solutions to other  problems (such as optimal control and reachable set estimation), analyzing systems with multiple time-delays, improving approximation quality by spatio-temporal partitioning \cite{Cibulka2021SpatioTemporalDO}, developing \ac{MV}-solutions for discrete-time systems with large time delays, handling graph-constrained history classes $\hs$ that have additional requirements (e.g., constant $x_h$ in time), and formulating \ac{MV}-solutions for \acp{DDE} with other types of time delays (e.g., proportional, distributed, unknown-but-bounded).

% Trajectory analysis problems with dynamic uncertainty may be phrased as optimal control problems, and bounding optimal control costs in time delay systems using occupation measures will be the subject of a sequel work.
% Uncertainties in delays (including time-evolving delays) will also be further examined.


==> sections/extensions.tex <==
% \section{Extensions}

\section{Sparsity Extension}
% \subsection{Delay Affine Structure}

\label{sec:delay_affine}

% A more general structure is when dynamics are affine in nonzero delays,
\urg{May send to arxiv copy in case we run out of room.}
Dynamics $f(t, x_0, \ldots, x_r)$ have \textit{current-delay-affine} structure if they can be separated into the following form,
\begin{equation}
\label{eq:dynamics_aff_non}
    \dot{x}(t) = \textstyle\sum_{i=1}^r f_i(t, x(t), x(t - \tau_i))
\end{equation}
The special structure of \eqref{eq:dynamics_aff_non} may be used to express weak solutions with measures in fewer variables \cite{lasserre2006convergent}. 

A correlative sparsity graph such as in \cite{waki2006sums} may be realized with $n + 1$ vertices corresponding to the variables $(t, x_0, x_1, \ldots, x_r)$. An edge is drawn between vertices if they appear in the same (non-additive) function. The Lie derivative term associated with \eqref{eq:dynamics_aff_non} is,
\begin{equation*}
    \Lie_f v(t, x_0) = \partial_t v(t, x_0) + \textstyle\sum_{i=1}^r f_i(t, x_0, x_i) \cdot \nabla_{x_0} v(t, x_0).
% \end{equation}
\end{equation*}

Under this definition, the cliques of the correlative sparsity graph are $(t, x_0, x_i)$ for all $i = 1, \ldots, r$ each corresponding to the term $f_i(t, x_0, x_i) \cdot \nabla_{x_0}v(t, x_0)$.
Joint occupation measures $\bar{\mu}^i \in \Mp{[0, T] \times X^2}$ may be defined on each clique, such that the overlapping marginal $\pi^{t x_0}_\# \bar{\mu}^i$ is identical for all cliques.
The decomposed Liouville constraint for all $v(t, x) \in C^1([0, T] \times X)$ is,
\begin{align}
\label{eq:liou_sparse}
    \inp{v(t, x)}{\mu_p} &= v(0, x_h(0)) + \inp{\partial_t v(t, x_0)}{\bar{\mu}^1} \\
    &+ \textstyle \sum_{i=1}^r\inp{f_i(t, x_0, x_1) \cdot v(t, x_0)}{\bar{\mu}^i}.\nonumber
\end{align}

The sparse consistency constraints for $i=1, \ldots, r$ with test functions $\phi_i(t, x) \in C([0, T], \times X)$ are,
\begin{align}
     \inp{\phi_i(t, x_i)}{\bar{\mu}^i} &= \textstyle \int_{t=-\tau_i}^0 \phi_i(t, x_h(t+\tau_i)) dt \\
     &+  \inp{\phi_i(t+\tau_i,x)}{\textstyle \sum_{j=-i}^{r-i} \nu_j }.\nonumber
\end{align}

The zero-lag consistency constraint also pins the marginal overlaps between joint occupation measures $\forall \phi_0 \in C([0, T] \times X), i =1, \ldots, r$,
\begin{align}
    \inp{ \phi_0(t, x_0)}{\bar{\mu}^i} &= \inp{\phi_0(t, x)}{\textstyle\sum_{j=0}^{r} \nu_j} .
\end{align}

With the correlatively sparse decomposition, the number of variables has dropped from $[1+n(r+1)]$ in $\bar{\mu}$ to $[1+2n]$ in $\bar{\mu_i} \ \forall i = 1, \ldots, r$. The complexity of \acp{LMI} generated from these measures correspondingly decrease in a polynomial manner as the number of variables in the largest measure falls.
\urg{will need a demo showing the timing impact}
% \subsection{Uncertainty}
% \urg{Briefly mention time-dependent and time-independent uncertainty, analogous to \cite{miller2021uncertain}.This uncertainty is an instance of an adversarial optimal control problem. Bounding optimal control costs in time delay systems using occupation measures will be the subject of a sequel work.}

==> sections/numerical_examples.tex <==
\section{Numerical Examples}
\label{sec:examples}
All experiments were developed in MATLAB 2021a, and code is available at \url{https://github.com/Jarmill/time_delay}. Dependencies include Gloptipoly \cite{henrion2003gloptipoly}, YALMIP \cite{Lofberg2004}, and Mosek \cite{mosek92} in order to formulate and solve \acp{LMI}. 

In this section, a notational convention where $(x_1, x_2)$ correspond to coordinates of $x \in X$ will be used.

% \urg{I will need to write a more comprehensive sampler to generate trajectories}

% \subsection{Peak Estimation}

% \section{Examples of Peak Estimation for Time-Delay Systems}

\label{sec:delay_traj_analysis_peak_example}

% \urg{Load in the peak estimation figures from the BrainPOP presentation.}

% % \subsection{Epidemic Model}
% This section provides an example of a weak solution and peak estimation given a single history in a compartmental epidemic model.
% Many diseases have incubation periods, in which there is a delay between initial infection and infectious potential. In the current COVID-19 pandemic, this incubation period appears to be between 2-14 days.  The epidemic  dynamics with time delays are, 
% \begin{subequations}
% \label{eq:sir_delay}
% \begin{align}
%     S'(t) &= -\beta S(t) I(t) \\
%     I'(t) &= \beta S(t-\tau) I(t-\tau) - \gamma I(t) \\
%     R'(t) &= \gamma I(t)
% \end{align}
% \end{subequations}
% There exists also exists a `latent' state $L'(t) = \beta S(t) I(t) - \beta  S(t - \tau) I (t - \tau)$ such that $S + I + R + L = 1$. The setting discussed in this section is $\beta = 0.4, \ \gamma = 0.1, \ \tau = 9, \ T = 30$ (9 day incubation period). A  constant history is assumed where $S(t) = 1-I_h, I(t) = I_h, R(t) = 0$ between $t \in [-9, 0]$ days for an initial infection rate of $I_h = 0.2$.
% For numerical purposes the dynamics are scaled such that $\tilde{t} \in [0, 1]$ with an effective delay of $\tilde{\tau} = \tau / T = 0.3$.
% Only the $x = (S, I)$ subsystem is considered with $\{S \geq 0, I \geq 0, S+I \leq 1\}$, and the joint occupation measure $\bar{\mu}$ has variables  $(t, S_0, I_0, S_1, I_1)$. 

% % Given a monomial $t^\beta S^{\alpha_1} I^{\alpha_2}$, the LMI estimated moment is $\hat{\mathbf{m}}_{\alpha \beta}: \inp{t^\beta S^{\alpha_1} I^{\alpha_2}}{\bar{\mu}}$.
% % The reference moments $\mathbf{m}_{\alpha \beta} = \int_{\tilde{t}=0}^1 (\tilde{t})^\beta S(T \tilde{t})^{\alpha_1} I(T \tilde{t})^{\alpha_2} d\tilde{t}$ were calculated by Simpson's rule on 1000 equally spaced points in $\tilde{t} \in [0, 1]$.
% % Figure \ref{fig:sir_weak} shows errors $\abs{\mathbf{m}_{\alpha \beta} - \hat{\mathbf{m}}_{\alpha \beta}}$ in LMI moment approximations to the trajectory from times $\tilde{t} \in [0, 1]$, indexed as the monomial powers increase $(\alpha, \beta)$ in a graded lexicographical order w.r.t $(\tilde{T}, S, I)$. 
% % The largest PSD block at order-3 has size 126, and at order-4 the largest PSD block has size 252.

% % \begin{figure}[h]
% % \centering
% %      \begin{subfigure}[b]{0.48\linewidth}
% %          \centering
% %          \includegraphics[width=\linewidth]{fig/sir_3_mom_approx.pdf}
% %          \caption{Order-3 moments, 2-norm$= 1.3062\times 10^{-4}$. }
% %          \label{fig:sir_weak_3}
% %      \end{subfigure}
% %      \;
% %      \begin{subfigure}[b]{0.48\linewidth}
% %          \centering
% %          \includegraphics[width=\linewidth]{fig/sir_4_mom_approx.pdf}
% %          \caption{Order-4 moments, 2-norm $= 4.2534 \times 10^{-5}$}
% %          \label{fig:sir_weak_4}
% %      \end{subfigure}
% %       \caption{\label{fig:sir_weak} Error in moment approximation}
% % \end{figure}

% Peak estimation is employed to bound the maximum infection rate over the course of the epidemic. This peak estimation program maximizes $\inp{I}{\mu_p}$ under the constraint that $(\mu_p, \bar{\mu}, \{\nu_0, \nu_1\}, \hat{\nu}_1)$ is a free-time weak solution of dynamics \eqref{eq:sir_delay}.

% Figure \ref{fig:sir_peak} displays the output of peak estimation, where the order-3 LMI relaxation bounds the maximal infection rate at 56.89\%. The moment matrix $\M_3[y_p]$ is approximately rank-1 (second largest eigenvalue of $\M_3[y_p] = 2.448\times 10^{-5}$), and the extracted optimum from $\M_3[y_p]$ by Algorithm 1 of \cite{miller2020recovery} is $(S^*, I^*) = (0.0561, 0.5689)$ occurring at $t^*=15.636$ days.
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.6\linewidth]{fig/sir_3_peak_traj2.pdf}
%     \caption{\label{fig:sir_peak} SIR Peak estimation at order 3}
    
% \end{figure}
\subsection{Delayed Flow System}

A time-delayed version of the Flow system dynamics from \cite{prajna2004safety} is
\begin{equation}
\label{eq:flow_delay}
    \dot{x}(t) = \begin{bmatrix}x_2(t) \\ -x_1(t-\tau) - x_2(t) + x_1(t)^3/3
        \end{bmatrix}.
\end{equation}

Figure \ref{fig:flow_delay_comparision} plots the delayed Flow system \eqref{eq:flow_delay} without lag ($\tau=0$ in blue) and with a lag ($\tau=0.75$ in orange) starting from the constant initial history $x_h(t) = [1.5, 0], \ \forall t \in [-\tau, 0]$ (black circle). 
% The system with lag spirals 
    \begin{figure}[ht]
        \centering
        \includegraphics[width=0.8\linewidth]{fig/flow_constant_compare.pdf}
        \caption{\label{fig:flow_delay_comparision}Comparison of delayed Flow systems \eqref{eq:flow_delay} with lags $\tau=0$ and $\tau= 0.75$ in times $t \in [0, 20]$}
    \end{figure}
    


The time-zero set of allowable histories is $X_0 = \{x \in \R^2 \mid  \ (x_1-1.5)^2 + x_2^2 \leq 0.4^2\}$. The history class $\hs$ will be the set of functions $x_h \in PC([-\tau, 0])$ whose graphs $(t, x(t))$ are contained within  the cylinder $H_0 = [-0.75, 0] \times X_0$. No further requirements of continuity are posed on histories in $\hs$.     
The considered peak estimation aims to find the minimum value of $x_2$ (maximize $p(x)=-x_2)$
for trajectories following \eqref{eq:flow_delay} starting from $H_0$, within the state set 
$X = [-1.25, 2.5] \times [-1.25, 1.5]$ and time horizon $T=5$. The first five bounds on the maximum value of $-x_2$ by solving \eqref{eq:peak_delay_lmi} are $p^*_{1:5}=[1.25, 1.2183, 1.1913, 1.1727, 1.1630]$.

Figure \ref{fig:flow_delay_peak} plots trajectories and peak information associated with this example. The black circle is the initial set $X_0$. The initial histories inside $X_0$ are plotted in grey. These sampled histories are piecewise constant with 10 uniformly spaced jumps (moving to a new point uniformly sampled in $X_0$) within $[-0.75, 0]$. The cyan curves are the \ac{DDE} trajectories of \eqref{eq:flow_delay} starting from the grey histories. The red dotted line is the $p^*_5$ bound on the minimum vertical coordinate of a point on any trajectory starting from $\hs$ up to a time horizon of $T=5$.
    \begin{figure}[ht]
        \centering
        \includegraphics[width=0.8\linewidth]{fig/peak_flow_5_T_5.png}
        \caption{\label{fig:flow_delay_peak} Minimize $x_2$ on the delayed Flow system \eqref{eq:flow_delay}}
    \end{figure}
    
    
    % Future work will involve more examples of peak estimation in time-delay systems.
    
    \subsection{Delayed Time-Varying System}
    
    This example involves peak estimation of \iac{DDE} version of the time-varying Example 2.1 of \cite{fantuzzi2020bounding}
    \begin{equation}
\label{eq:time_var_delay}
    \dot{x}(t) = \begin{bmatrix}x_2(t) t - 0.1 x_1(t) - x_1(t-\tau) x_2(t-\tau)  \\ -x_1(t) t - x_2(t) + x_1(t) x_1(t-\tau)
        \end{bmatrix}.
\end{equation}

The considered support parameters are $\tau = 0.75, \ T = 5, $ and $X = [-1.25, 1.25] \times [-0.75, 1.25]$. Figure \ref{fig:time_var_delay_hist} plots four different sets of trajectories of \eqref{eq:time_var_delay} originating from different history classes. For convenience, define the disc set $X_\bullet$ as $\{x\in \R^2 \mid (x_1+0.75)^2 + x_2^2 \leq 0.3^2\}$ and the center-point of the disc $X_\bullet$ as $C_0 = [0.75; 0]$. 
The top-left plot (Free) has a history class $\hs$ in which the time-zero set is the disk $X_0 = X_\bullet$ and the graphs of the histories are contained inside $H_0 = [-0.75, 0] \times X_0$. The bottom-left plot (Constant) additionally requires that the trajectories in $H_0$ should be constant (as imposed by a shaping constraint from Section \ref{sec:shaping}).
The top-right plot (Pinhole) has $X_0 = [0; 0.75]$ and $H_0 = ([-0.75, 0) \times X_\bullet)\cup (\{0\} \times C_0)$, such that all trajectories pass through the point $X_0 = C_0$ at time $t=0^+$. The bottom-right plot (Constant-Center Jump) is the opposite of (Pinhole), in which the history set is $H_0 = ([-0.75, 0) \times C_0)\cup ((0) \times X_\bullet)$ and $X_0 = X_\bullet$.

dddddddddd


% The time-zero set is the disk $X_0 = \{x\in \R^2 \mid (x_1+0.75)^2 + x_2^2 \leq 0.3^2\}$. The only restriction on allowable histories $\hs$ is that their graphs are contained in the history set $H_0 = [-0.75, 0] \times X_0$. 

Solving the \ac{SDP} associated with the \ac{LMI} \eqref{eq:peak_delay_lmi}  in the (Free) setting to maximize $p(x) = x_1$ yields bounds $p^*_{1:5} = [1.25, 1.25, 1.1978, 0.8543, 0.7183].$  The (Constant) setting with shaping constraints results in $p^*_{1:4} = [1.25, 1.25,1.009, 0.6943].$ The (Pinhole) problem with $\mu_h \in \Mp{[-0.75, 0] \times X_\bullet}$ yields $p^*_{1:3}=[1.25, 1.25, 0.5598]$, and its opposite (Constant-Center Jump) setting with $\mu_h \in \Mp{[-0.75, 0] \times C_0}$ results in $p^*_{1:3}=[1.25, 1.25, 0.6464]$. Higher order \ac{LMI} relaxations than depicted lead to degraded conditioning and invalid bounds. Partitioning \cite{Cibulka2021SpatioTemporalDO} and numerically stable bases (e.g. Chebyshev) may lead to improved approximation capacity.


Figure \ref{fig:time_var_peak} plots system trajectories and the $p^*_5$ bound on $x_1$ using the same visual convention as Figure \ref{fig:time_var_peak} (black circle $X_0$, grey histories $x_h(t)$, cyan trajectories $x(t \mid x_h)$, red dotted line $x_1 = p^*_5$).

    \begin{figure}[ht]
        \centering
        \includegraphics[width=0.8\linewidth]{fig/peak_time_var_5.png}
        \caption{\label{fig:time_var_peak} Maximize $x_1$ on the delayed time-varying \eqref{eq:time_var_delay}}
    \end{figure}

% Figure \ref{fig:time_var_peak_3d} plots the trajectory and bound information of \ref{fig:time_var_peak} in 3d $(t, x_1, x_2)$. The history structure inside $H_0$ between times $[-0.75, 1]$ is clearly visible in grey.



    %     \begin{figure}[ht]
    %     \centering
    %     \includegraphics[width=\linewidth]{fig/peak_time_var_3d.png}
    %     \caption{\label{fig:time_var_peak_3d} A 3d plot of \eqref{eq:time_var_delay} and its  $x_1$ bound }
    % \end{figure}

% Peak estimation of $p(x) = x_2$ under the same system parameters leads to the bounds $p^*_{1:5} = [1.25, 1.25, 0.9557, 0.9138, 0.9112].$ 

==> sections/numerical_examples_std.tex <==
\section{Numerical Examples}
\label{sec:examples}
All experiments were developed in MATLAB 2021a, and code is available at  \url{https://github.com/Jarmill/timedelay}. 
Dependencies include Gloptipoly \cite{henrion2003gloptipoly}, YALMIP \cite{Lofberg2004}, and Mosek \cite{mosek92} in order to formulate and solve moment-\ac{SOS} \acp{LMI} and \acp{SDP}. 

In this section, a notational convention where $(x_1, x_2)$ correspond to coordinates of $x \in X$ will be used. All sampled histories in visualizations are piecewise-constant inside $H_0$ with 10 randomly-spaced jumps between $[-\tau, 0]$.

% \urg{I will need to write a more comprehensive sampler to generate trajectories}

% \subsection{Peak Estimation}

% \section{Examples of Peak Estimation for Time-Delay Systems}

\label{sec:delay_traj_analysis_peak_example}

% \urg{Load in the peak estimation figures from the BrainPOP presentation.}

% % \subsection{Epidemic Model}
% This section provides an example of a weak solution and peak estimation given a single history in a compartmental epidemic model.
% Many diseases have incubation periods, in which there is a delay between initial infection and infectious potential. In the current COVID-19 pandemic, this incubation period appears to be between 2-14 days.  The epidemic  dynamics with time delays are, 
% \begin{subequations}
% \label{eq:sir_delay}
% \begin{align}
%     S'(t) &= -\beta S(t) I(t) \\
%     I'(t) &= \beta S(t-\tau) I(t-\tau) - \gamma I(t) \\
%     R'(t) &= \gamma I(t)
% \end{align}
% \end{subequations}
% There exists also exists a `latent' state $L'(t) = \beta S(t) I(t) - \beta  S(t - \tau) I (t - \tau)$ such that $S + I + R + L = 1$. The setting discussed in this section is $\beta = 0.4, \ \gamma = 0.1, \ \tau = 9, \ T = 30$ (9 day incubation period). A  constant history is assumed where $S(t) = 1-I_h, I(t) = I_h, R(t) = 0$ between $t \in [-9, 0]$ days for an initial infection rate of $I_h = 0.2$.
% For numerical purposes the dynamics are scaled such that $\tilde{t} \in [0, 1]$ with an effective delay of $\tilde{\tau} = \tau / T = 0.3$.
% Only the $x = (S, I)$ subsystem is considered with $\{S \geq 0, I \geq 0, S+I \leq 1\}$, and the joint occupation measure $\bar{\mu}$ has variables  $(t, S_0, I_0, S_1, I_1)$. 

% % Given a monomial $t^\beta S^{\alpha_1} I^{\alpha_2}$, the LMI estimated moment is $\hat{\mathbf{m}}_{\alpha \beta}: \inp{t^\beta S^{\alpha_1} I^{\alpha_2}}{\bar{\mu}}$.
% % The reference moments $\mathbf{m}_{\alpha \beta} = \int_{\tilde{t}=0}^1 (\tilde{t})^\beta S(T \tilde{t})^{\alpha_1} I(T \tilde{t})^{\alpha_2} d\tilde{t}$ were calculated by Simpson's rule on 1000 equally spaced points in $\tilde{t} \in [0, 1]$.
% % Figure \ref{fig:sir_weak} shows errors $\abs{\mathbf{m}_{\alpha \beta} - \hat{\mathbf{m}}_{\alpha \beta}}$ in LMI moment approximations to the trajectory from times $\tilde{t} \in [0, 1]$, indexed as the monomial powers increase $(\alpha, \beta)$ in a graded lexicographical order w.r.t $(\tilde{T}, S, I)$. 
% % The largest PSD block at order-3 has size 126, and at order-4 the largest PSD block has size 252.

% % \begin{figure}[h]
% % \centering
% %      \begin{subfigure}[b]{0.48\linewidth}
% %          \centering
% %          \includegraphics[width=\linewidth]{fig/sir_3_mom_approx.pdf}
% %          \caption{Order-3 moments, 2-norm$= 1.3062\times 10^{-4}$. }
% %          \label{fig:sir_weak_3}
% %      \end{subfigure}
% %      \;
% %      \begin{subfigure}[b]{0.48\linewidth}
% %          \centering
% %          \includegraphics[width=\linewidth]{fig/sir_4_mom_approx.pdf}
% %          \caption{Order-4 moments, 2-norm $= 4.2534 \times 10^{-5}$}
% %          \label{fig:sir_weak_4}
% %      \end{subfigure}
% %       \caption{\label{fig:sir_weak} Error in moment approximation}
% % \end{figure}

% Peak estimation is employed to bound the maximum infection rate over the course of the epidemic. This peak estimation program maximizes $\inp{I}{\mu_p}$ under the constraint that $(\mu_p, \bar{\mu}, \{\nu_0, \nu_1\}, \hat{\nu}_1)$ is a free-time weak solution of dynamics \eqref{eq:sir_delay}.

% Figure \ref{fig:sir_peak} displays the output of peak estimation, where the order-3 LMI relaxation bounds the maximal infection rate at 56.89\%. The moment matrix $\M_3[y_p]$ is approximately rank-1 (second largest eigenvalue of $\M_3[y_p] = 2.448\times 10^{-5}$), and the extracted optimum from $\M_3[y_p]$ by Algorithm 1 of \cite{miller2020recovery} is $(S^*, I^*) = (0.0561, 0.5689)$ occurring at $t^*=15.636$ days.
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.6\linewidth]{fig/sir_3_peak_traj2.pdf}
%     \caption{\label{fig:sir_peak} SIR Peak estimation at order 3}
    
% \end{figure}
\subsection{Delayed Flow System}

A time-delayed version of the Flow system from \cite{prajna2004safety} is
\begin{equation}
\label{eq:flow_delay}
    \dot{x}(t) = \begin{bmatrix}x_2(t) \\ -x_1(t-\tau) - x_2(t) + x_1(t)^3/3
        \end{bmatrix}.
\end{equation}

Figure \ref{fig:flow_delay_comparision} plots the delayed Flow system \eqref{eq:flow_delay} without lag ($\tau=0$ in blue) and with a lag ($\tau=0.75$ in orange) starting from the constant initial history $x_h(t) = (1.5, 0), \ \forall t \in [-\tau, 0]$ (black circle). 
% The system with lag spirals 
    \begin{figure}[ht]
        \centering
        \includegraphics[width=0.8\linewidth]{fig/flow_constant_compare.pdf}
        \caption{\label{fig:flow_delay_comparision}Comparison of delayed Flow systems \eqref{eq:flow_delay} with lags $\tau=0$ and $\tau= 0.75$ in times $t \in [0, 20]$ }
    \end{figure}
    


The time-zero set of allowable histories is $X_0 = \{x \in \R^2 \mid  \ (x_1-1.5)^2 + x_2^2 \leq 0.4^2\}$. The history class $\hs$ will be the set of functions $x_h \in PC([-\tau, 0])$ whose graphs $(t, x(t))$ are contained within  the cylinder $H_0 = [-0.75, 0] \times X_0$. No further requirements of continuity are posed on histories in $\hs$.     
The considered peak estimation aims to find the minimum value of $x_2$ (maximize $p(x)=-x_2)$
for trajectories following \eqref{eq:flow_delay} starting from $H_0$, within the state set 
$X = [-1.25, 2.5] \times [-1.25, 1.5]$ and time horizon $T=5$. The first five bounds on the maximum value of $-x_2$ by solving \eqref{eq:peak_delay_lmi} are $p^*_{1:5}=[1.25, 1.2183, 1.1913, 1.1727, 1.1630]$.

Figure \ref{fig:flow_delay_peak} plots trajectories and peak information associated with this example. The black circle is the initial set $X_0$. The initial histories inside $X_0$ are plotted in grey. These sampled histories are piecewise constant with 10 uniformly spaced jumps (moving to a new point uniformly sampled in $X_0$) within $[-0.75, 0]$. The cyan curves are the \ac{DDE} trajectories of \eqref{eq:flow_delay} starting from the grey histories. The red dotted line is the $p^*_5$ bound on the minimum vertical coordinate of a point on any trajectory starting from $\hs$ up to $T=5$.
    \begin{figure}[ht]
        \centering
        \includegraphics[width=0.8\linewidth]{fig/peak_flow_5_T_5.png}
        \caption{\label{fig:flow_delay_peak} Minimize $x_2$ on the delayed Flow system \eqref{eq:flow_delay}}
    \end{figure}
    
    
    % Future work will involve more examples of peak estimation in time-delay systems.
    
    \subsection{Delayed Time-Varying System}
    
    This example involves peak estimation of \iac{DDE} version of the time-varying Example 2.1 of \cite{fantuzzi2020bounding}
    \begin{equation}
\label{eq:time_var_delay}
    \dot{x}(t) = \begin{bmatrix}x_2(t) t - 0.1 x_1(t) - x_1(t-\tau) x_2(t-\tau)  \\ -x_1(t) t - x_2(t) + x_1(t) x_1(t-\tau)
        \end{bmatrix}.
\end{equation}

The considered support parameters are $\tau = 0.75, \ T = 5, $ and $X = [-1.25, 1.25] \times [-0.75, 1.25]$.
The time-zero set is the disk $X_0 = \{x\in \R^2 \mid (x_1+0.75)^2 + x_2^2 \leq 0.3^2\}$. The only restriction on allowable histories $\hs$ is that their graphs are contained in the history set $H_0 = [-0.75, 0] \times X_0$. 

Solving the \ac{SDP} associated with the \ac{LMI} \eqref{eq:peak_delay_lmi} to maximize the peak function $p = x_1$ yields the sequence of five bounds $p^*_{1:5} = [1.25, 1.25, 1.1978, 0.8543, 0.718264618]$. 
Figure \ref{fig:time_var_peak} plots system trajectories and the $p^*_5$ bound on $x_1$ using the same visual convention as Figure \ref{fig:flow_delay_peak} (black circle $X_0$, grey histories $x_h(t)$, cyan trajectories $x(t \mid x_h)$, red dotted line $x_1 = p^*_5$).

    \begin{figure}[ht]
        \centering
        \includegraphics[width=0.8\linewidth]{fig/peak_time_var_5.png}
        \caption{\label{fig:time_var_peak} Maximize $x_1$ on the delayed time-varying \eqref{eq:time_var_delay}}
    \end{figure}

Figure \ref{fig:time_var_peak_3d} plots the corresponding trajectory and bound information in 3d $(t, x_1, x_2)$. The black circles denote the boundary of $H_0$. The history structure inside $H_0$ between times $[-0.75, 1]$ is clearly visible in grey.

        \begin{figure}[ht]
        \centering
        \includegraphics[width=\linewidth]{fig/time_var_3d_hist_circ.png}
        \caption{\label{fig:time_var_peak_3d} A 3d plot of \eqref{eq:time_var_delay} and its  $x_1$ bound }
    \end{figure}

The peak estimation of $p = x_2$ under the same system parameters leads to the sequence of five bounds $p^*_{1:5} = [1.25, 1.25, 0.9557, 0.9138, 0.9112].$ 

==> sections/peak.tex <==
\section{Peak Estimation of DDEs}
\urg{ Revise and Excise this content}
% \section{Peak Estimation of Time-Delay Systems}

% Free-terminal time weak solutions may be employed to produce upper bounds on the peak estimation problem \eqref{eq:peak_delay_traj}.

\subsection{Measure Program}

Problem \eqref{eq:peak_delay_traj} may be upper-bounded by a measure \ac{LP} program to produce an objective $p^* \geq P^*$. This measure program is based on the multiple-history free-time weak solution $(\mu_0, \mu_T, \bar{\mu}, \{\nu_j\}_{j=-r}^r, \{\hat{\nu_i}\}_{i=1}^r)$ from Definition \ref{defn:weak_multiple_free} (with the convention that $\hat{\nu}_0 = 0$),

\begin{subequations}
\label{eq:peak_delay_meas}
\begin{align}
p^* = & \ \textrm{max} \quad \inp{p(x)}{\mu_p} \label{eq:peak_delay_meas_obj} \\
    & \mu_p = \delta_0 \otimes \mu_0 + \pi^{tx_0}_\# \Lie_f^\dagger \bar{\mu} \label{eq:peak_delay_meas_flow}\\
    & \inp{1}{\mu_0} = 1 \label{eq:peak_delay_meas_prob}\\
    & \pi^{t x_i}_\# \bar{\mu} + \hat{\nu}_i = (t + \tau_i, x)_\# \left( \textstyle\sum_{j=-i}^{r-i} \nu_{j} \right) & & \forall i = 0, \ldots, r \label{eq:peak_delay_meas_delay} \\
    & \pi^t_\# \left( \textstyle\sum_{i=1}^r \nu_{-i} \right) = \lambda_{[-\tau_r, 0]} \label{eq:peak_delay_meas_history} \\
    & \mu_0 \in \Mp{X_0} \label{eq:peak_delay_meas_init} \\
    & \mu_p \in \Mp{[0, T] \times X} \label{eq:peak_delay_meas_peak}\\
    & \bar{\mu} \in \Mp{[0, T] \times X^{r+1}} \label{eq:peak_delay_meas_occ} \\
    &\nu_{j} \in \Mp{\Omega_j} & &  \forall j = -r, \ldots, r \\
    & \hat{\nu}_i \in \Mp{[0, T] \times X} \label{eq:peak_delay_meas_complement}& &  \forall i = 1, \ldots, r.
\end{align}
\end{subequations}
 

Constraint \eqref{eq:peak_delay_meas_delay} is an equivalent (weak) expression to the free-time multiple-history consistency constraint in \eqref{eq:consistency_multi_free}. Shaping constraints may optionally be added as per Section \ref{sec:shaping} to describe valid trajectories in the function class $\mathcal{H}$.

For $r$ time-delays and $n$ states, there will be 1 measure with $(r+1)n + 1$ variables ($\mu$), $3r-1$ measures with $n+1$ variables (in order: components $\nu_{i}$, complements $\hat{\nu}_{i}$ from absolute continuity of components, and $\mu_p$), and 1 measure of size $n$ ($\mu_0$). LMI relaxations of program \eqref{eq:peak_delay_meas} will scale combinatorially with the number of delay terms $r$, and the bottleneck in optimization will be the joint occupation measure $\bar{\mu}$. 
 
\subsection{Function Program}
Dual variables must be introduced to formulate the Lagrangian of problem \eqref{eq:peak_delay_meas}. Let $v(t,x) \in C^1([0, T] \times X), \ \gamma \in \R, \  \phi_i(t, x_i) \in C([0, T] \times X) \ \forall i = 0, \ldots, r,$ and $h(t) \in C([-\tau_r, 0])$ be dual variables for constraints \eqref{eq:peak_delay_meas_flow}-\eqref{eq:peak_delay_meas_delay}. 
The Lagrangian of problem \eqref{eq:peak_delay_meas} is,

\begin{align}
    \scL &= \inp{p(x)}{\mu_p} + \inp{v(t,x_0)}{\delta_0 \otimes \mu_0 + \pi^{t x_0}_\# \Lie_f^\dagger \bar{\mu} - \mu_p} + \gamma(1 - \inp{1}{\mu_0})\\\label{eq:peak_lagrangian}
    & + \textstyle \sum_{i=0}^r \inp{\phi_i(t, x)}{\pi^{t x_i}_\# \bar{\mu} + \hat{\nu}_i -(t + \tau_i, x)_\# \left( \textstyle\sum_{j=-i}^{r-i} \nu_{j} \right)} + \inp{h(t)}{\lambda_{[-\tau_r, 0]} - \left(\textstyle\sum_{i=1}^r \nu_{-i} \right) }. \nonumber
\end{align}

The dual problem (function program) of \eqref{eq:peak_delay_meas} formed by taking a saddle point to $\scL$ is,
\begin{subequations}
\label{eq:peak_delay_cont}
\begin{align}
    d^* = & \ \min_{\gamma + \in \R} \gamma + \textstyle \int_{t=-\tau_r}^0 h(t) dt & & \\
    & \gamma \geq v(0, x)  & & \forall x \in  X_0 \label{eq:peak_delay_cont_init}\\
    & v(t, x) \geq p(x) & & \forall (t, x) \in [0, T] \times X \label{eq:peak_delay_cont_p} \\
    & 0 \geq \Lie_f v(t, x_0) + \textstyle \sum_{i=0}^{r} \phi_i(t, x_i)& & \forall (t, \cup_{i=0}^r x_i)\in [0, T] \times X^{r+1} \\
    & \phi_i(t, x) \leq 0 & & \forall (t, x) \in \Omega_{i}, \ i = 1, \ldots, r \\ 
    & \textstyle \sum_{i=j}^{r} \phi_i(t + \tau_i, x) \geq 0 & & \forall (t, x) \in \Omega_j, \ j = 0, \ldots, r \\
    & \textstyle\sum_{i=0}^{r-j} \phi_i(t + \tau_i, x)  + h(t)\geq 0 & & \forall (t, x) \in \Omega_{-j}, \ j = 1, \ldots, r \\
    & v(t,x) \in C^1([0, T]\times X) \label{eq:peak_delay_cont_v}& & \\
    &\phi_i(t, x) \in C([0, T] \times X) & &  \forall i=0, \ldots, r \label{eq:peak_delay_cont_phi} \\
    &h(t) \in C([-\tau_r, 0]).
\end{align}
\end{subequations}
The variable $v(t, x)$ is an auxiliary function that upper bounds the cost $p(x)$ over the area of interest $[0, T] \times X$. The $\phi_i$ terms are introduced by delay dynamics, and the $h(t)$ function is required to ensure the  sanctity of histories (Lebesgue marginal in time). Without time-delays, this problem is equal to the standard peak estimation measure formulation because the multipliers $\phi_i(t, x)$ will be set to $0$. 

Problems \eqref{eq:peak_delay_meas} and \eqref{eq:peak_delay_cont} achieve strong duality such that $p^* = d^*$ when the set $[-\tau_r, T] \times X$ is compact by Theorem 3.10 of \cite{anderson1987linear} \urg{write in appendix, send to Arxiv}. 
The measures in problem \eqref{eq:peak_delay_meas} form a free-time multiple-history weak solution and therefore have bounded mass when the set $[-\tau_r, T] \times X$ is compact. The constraints defining this weak solution are closed in the weak-$*$ topology, so the conditions for strong duality by Theorem 3.10 of \cite{anderson1987linear} are therefore satisfied.



==> sections/preliminaries.tex <==
\section{Preliminaries}
\label{sec:preliminaries}
% \subsection{Acronyms/Initialisms}
\input{sections/acronym}

\subsection{Notation}

The $n$-dimensional real Euclidean vector space is $\R^n$. The set of natural numbers is $\N$, and the set of $n$-dimensional multi-indices is $\N^n$. The degree of a multi-index $\alpha \in \N^n$ is $\abs{\alpha} = \sum_{i=1}^n \alpha_i$.
The set of polynomials with real coefficients in an indeterminate $x$ is $\R[x]$. Each polynomial $p(x) \in \R[x]$ has a unique representation in terms of a finite index set $\mathcal{J} \subset \N^n$ and coefficients $\{p_\alpha\}_{\alpha \in \mathcal{J}}$ with $p_\alpha \neq 0$ as $p(x) = \sum_{\alpha \in \mathcal{J}} p_\alpha \left(\prod_{i=1}^n x_i^{\alpha_{i}}\right) = \sum_{\alpha \in \mathcal{J}} p_\alpha x^\alpha$. The degree of a polynomial $\deg p(x)$ is equal to $\max_{\alpha \in \mathcal{J}} \abs{\alpha_j}$. The subset of polynomials with degree at most $d$ is $\R[x]_{\leq d} \subset \R[x]$.

\subsection{Analysis and Measure Theory}
Let $X$ be a topological space.
The set of continuous functions over a space $X$ is $C(X)$, and its subcone of nonnegative functions over $X$ is $C_+(X)$. The subset of once-differentiable functions over $X$ is $C^1(X) \subset C(X)$. A single-variable function $g(t)$ is \ac{PC}  over the domain $[a, b]$ if there exist $B \in \N \backslash \{0\}$ and a finite number of time-breaks $t_0 = a < t_1 < t_2 <  \cdots < t_{B} < b = t_{B+1}$ such that the function $g(t)$ is continuous in each interval $[t_k, t_{k+1})$ for $k = 0..B$.
The class of \ac{PC} functions from the time interval $[-\tau, 0]$ to $X$ is $PC([-\tau, 0], X)$.

The set of nonnegative Borel measures over $X$ is $\Mp{X}$. A pairing exists between functions $p \in C(X)$ and measures $\mu \in \Mp{X}$ by Lebesgue integration with $\inp{p}{\mu} = \int_X p(x) d \mu(x)$. 
This pairing is a duality pairing and defines an inner product 
% \MK{Milan: This is typically not called inner product, just duality pairing. When  you say inner product, a (pre)-Hilbert structure is typically assumed, which we don't have here.} 
between $C_+(X)$ and $\Mp{X}$ when $X$ is compact. The $\mu$-measure of a set $A \subseteq X$ may be defined in terms of $A$'s indicator function ($I_A(x)=1$ if $x \in A$ and $I_A(x)=0$ otherwise) as $\mu(A) = \inp{I_A(x)}{\mu(x)}$. The quantity $\mu(X)$ is called the mass of $\mu$, and $\mu$ is a probability distribution if $\mu(X) = 1$. The support of $\mu$ is the set of all points $x$ such that all open neighborhoods $N_x \ni x$ satisfy $\mu(N_x) > 0$. 
Two special measures are the Dirac delta and the Lebesgue measure. The Dirac delta $\delta_{x}$ with respect to a point $x \in X$ obeys the point-evaluation pairing $\inp{p}{\delta_{x}} = p(x)$ for all $p \in C(X)$. The Lebesgue (volume) distribution has the definition $\inp{p}{\lambda_X} = \int_X p(x) dx$. Further details about measure theory are available in \cite{tao2011introduction}.

Given spaces $X$ and $Y$, the projection $\pi^x: X \times Y \rightarrow X$ is the map $(x, y) \mapsto x$.
For measures $\mu \in \Mp{X}$ and $\nu \in \Mp{Y}$, the product measure $\mu \otimes \nu \in \Mp{X \times Y}$ is the unique measure satisfying $(\mu\otimes \nu)(A \times B) = \mu(A)\nu(B)$ for all subsets $A \subseteq X, \ B \subseteq Y$. For two measures $\mu, \xi \in \Mp{X}$, the measure $\mu$ dominates $\xi$ ($\xi \leq \mu$) if $\xi(A) \leq \mu(A), \ \forall A \subset X$. To every dominated measure $\xi \leq \mu$ there exists a slack measure $\hat{\xi} \in \Mp{X}$ such that 
$\xi + \hat{\xi} = \mu$.

% and observe that $\hat\mu$ is nonnegative since $\xi \le \mu$.
% \MK{Milan: The notation $\xi \ll \mu$ is typically used to denote that $\xi$ is absolutely continuous wrt $\mu$, which is not equivalent to what's written here.} 
% \victor{It seems that this notation is never used.}
% By the Jordan decomposition, there exists a slack measure $\hat{\mu} \in \Mp{X}$ such that $\mu = \hat{\mu} + \xi$. \MK{Milan: The previous statement does not need a Jordan decomposition. Simply define $\hat \mu = \mu - \xi$ and observe that $\hat\mu$ is nonnegative since $\xi \le \mu$. }



The pushforward of a map $Q: X \rightarrow Y$ along a measure $\mu$ is $Q_\# \mu$, with the relation $\inp{z}{Q_\# \mu} = \inp{z \circ Q }{\mu}$ holding for all $z \in C(Y)$. Given $\eta \in \Mp{X \times Y}$, the projection-pushforward $\pi^x_\# \eta$ is the $x$-marginalization of $\eta$. The pairing of $p \in C(X)$ with $\pi^x_\#\eta$ may be equivalently expressed as $\inp{p}{\pi^x_\#\eta} = \inp{p}{\eta}$.
The adjoint of a linear map $\Lie: C(X)\rightarrow C(Y)$ is a mapping $\Lie^\dagger:M(Y)\to M(X)$ satisfying $\inp{\Lie p}{\nu} = \inp{p}{\Lie^\dagger \nu}$ for all $p \in C(X)$ and $\nu \in M(Y)$.

% \urg{Topics in Measures
% \begin{itemize}
%     \item Nonnegative Measure
%     \item Pushforwards and Marginalization
%     \item Absolute Continuity
% \end{itemize}}



\subsection{Time Delay Systems}


% \MK{Milan: Do we need PC in the next statement instead of Borel measurable?} 
Given a \ac{PC} state history $t \mapsto x_h(t), \ t \in [-\tau, 0]$,  a unique forward trajectory $x(t \mid x_h)$ of \eqref{eq:delay_dynamics} exists on  $t \in [0, T]$ if the function $(t,x_0,x_1) \mapsto f(t, x_0, x_1)$ is locally Lipschitz in all variables. Such locally Lipschitz dynamics satisfy a smoothing property: the order of trajectory time-derivatives that are continuous will increase by 1 every $\tau$ time steps \cite{fridman2014intro}. 
% \MK{Milan: Any reference to the last statement?}


% Trajectories of time-delay systems with the form of \eqref{eq:delay_dynamics} with $f$ (locally) Lipschitz satisfy a smoothing property as shown in Figure \ref{fig:increasing_continuity}. The order of derivatives that are continuous will increase by 1 every $\tau$ time steps. An example of such a time-delay system is visualized in Figure \ref{fig:increasing_continuity} with system dynamics,
% \begin{equation}
%     x'(t) = -2x(t)-2x(t-1). \label{eq:time_delay_fig}
% \end{equation} 
% The plotted histories are lines that pass through $x_h(0)=1$, and their evolution after time $t = 0$ is different.


% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.7\linewidth]{fig/increasing_continuity.pdf}
%     \caption{Continuity of \eqref{eq:time_delay_fig} trajectories increases every $\tau=1$ time step}
%     \label{fig:increasing_continuity}
% \end{figure}

The behavior of time-delay systems may change and bifurcate as the time delays change. A well-studied example of $\dot{x} = -x(t-\tau)$
% is plotted in Figure 
% \eqref{fig:stability_switch} \cite{fridman2014intro}, 
in which the system is stable (to $x=0$) for all bounded \ac{PC} histories with $\tau \in [0, \pi/2)$, has bounded oscillations for some initial histories at $\tau=\pi/2$ (e.g. constant $x_h$ in time), and is unstable (divergent oscillations to $\pm \infty$) for all similar histories with $\tau > \pi/2$ \cite{fridman2014intro}.

Problem \eqref{eq:peak_delay_traj} involves a class of histories $\hs$. In this paper, we will impose that $\hs$ is graph-constrained,
\begin{defn}
\label{defn:graph_constrained}
    The history class $\hs$ is \textbf{graph-constrained} if $\hs$ is the set of histories whose graph lies within a given set $H_0 \subseteq [-\tau, 0] \times X$,
\begin{align*}
    \hs = \{x_h \in PC([-\tau, 0], X) \mid (t, x_h(t)) \in H_0 \ \forall t \in [-\tau, 0]\},
\end{align*} 
and there are no other continuity restrictions on histories.
\end{defn}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.7\linewidth]{fig/stability_switch.pdf}
%     \caption{Bifurcation of stability as $\tau$ exceeds $\pi/2$ in $\dot{x}=-x(t-\tau)$}
%     \label{fig:stability_switch}
% \end{figure}

% \urg{Talk about classes of histories $\hs \in PC([-\tau, 0], X)$}


\subsection{Occupation Measures}

The \textbf{occupation measure} associated with an interval $[a, b]  \subset \R$ and a curve $t \mapsto x(t) \in PC([a, b], X)$ is the pushforward of the Lebesgue distribution (in time) $\lambda_{[a, b]}$ along the curve evaluation. 
Such an occupation measure $\mu_{x(\cdot)} \in \Mp{[a, b] \times X}$ satisfies a relation for all $v \in C([a, b] \times X):$
\begin{align}
    \inp{v}{\mu_{x(\cdot)}} & = \textstyle \int_{a}^b v(t, x(t)) dt.
\end{align}
% \MK{Milan: I would suggest the notation $\mu_{x(\cdot)}$ instead of $\mu_{(t, x(t))}$.}

% \MK{Milan: There is a jump in the thought process. You never speak about control and now it pops up out of the blue.} 

Occupation measures can be extended to controlled dynamics.
Let $U \subset \R^m$ be a set of input-values and define the following controlled dynamics (in which $u(t) \in U$ for all $t \in [0, T]$) 
\begin{align}
    \dot{x}(t) &= f(t, x(t), u(t)). \label{eq:dynamics_u}
\end{align}

The  occupation measure of a trajectory of \eqref{eq:dynamics_u} given a stopping time $t^*$, an initial condition $x_0 \in X_0 \subset X$ and a measurable  control $u(\cdot)$ (such that $u(t)$ is a probability distribution over $U$ for each $t \in [0, t^*]$) for sets $A \subseteq [0, T], \ B \subseteq X, \ C \subseteq U$ is
\begin{align}   
\label{eq:occ_free_single}
    &\mu(A \times B\times C \mid t^*, x_0) = \\
    &\int_{[0, t^*] \times X_0\times U} I_{A \times B \times C}\left((t, x(t \mid x_0,  u(\cdot)), u(t)\right) dt. \nonumber
\end{align}
% \MK{Milan: $\mathcal{U}$ is not properly defined. Also, why is $u$ in a feedback form in \eqref{eq:occ_free_single}? Normally it is required to depend only on time.}

The occupation measure in \eqref{eq:occ_free_single} may be averaged over a distribution of initial conditions  $\mu_0(x_0)$,
\begin{align}
    \label{eq:avg_free_occ}
    &\mu(A \times B\times C \mid t^*) = \\
    &\int_{X_0} \mu(A \times B\times C \mid t^*, x_0) d\mu_0(x_0). \nonumber
\end{align}

% is defined with respect to 
% $\tilde{v} \in C([0, T] \times X \times U):$
% \begin{align}
%  % \label{eq:avg_free_occ}
%     \inp{\tilde{v}}{\mu_{(t, x(t), u(t))}} & = \textstyle \int_{a}^b \tilde{v}(t, x(t), u(t)) dt.
% \end{align}

% A free-terminal-time averaged occupation measure posed over a stopping time $t^* \in [0, T]$, a control $u(\cdot) \in \mathcal{U}$, and a distribution of initial conditions $\mu_0$ is,



% \urg{Is this definition correct? There must be an easier way to phrase this, such as in Section 3.1 of \cite{henrion2013convex}.}

% \MK{Define the Lie derivative $\Lie$ of a function $v \in C^1([-\tau,T]\times \R^n)$  along~\eqref{eq:dynamics_u} by}
A linear operator $\Lie_f$ may be defined for every $v \in C^1([-\tau,T]\times \R^n)$ by
\begin{equation}
\label{eq:lie}
    \Lie_f v(t, x) = \partial_t v(t,x) + f(t,x, u) \cdot \nabla_x v(t,x).
\end{equation}
% \MK{Note that $\Lie_f$ is a linear operator}. \MK{Milan: I probably wouldn't call $\Lie_f$ a Lie derivative. }
A distribution of initial conditions $\mu_0 \in \Mp{X_0}$, free-terminal-time values $\mu_p \in \Mp{[0, T] \times X}$, and occupation measures $\mu \in \Mp{[0, T] \times X \times U}$ from \eqref{eq:avg_free_occ} are connected together by Liouville's equation for all $v \in C^1([0, T] \times X)$
\begin{subequations}
\label{eq:liou}
\begin{align}
\inp{v}{\mu_p} &= \inp{v(0, x)}{\mu_0(x)} + \inp{\Lie_f v}{\mu} \label{eq:liou_int}\\
\mu_p &= \delta_0 \otimes \mu_0 + \pi^{t x}_\# \Lie_f^\dagger \mu. \label{eq:liou_weak}
\end{align}
\end{subequations}
Equation \eqref{eq:liou_weak} is a shorthand notation for \eqref{eq:liou_int} when applied to all $C^1$  functions $v$. Note that the $\pi^{t x}_\#$ marginalizes out the input $u$ in the occupation measure $\mu$. Any $\mu$ as part of a tuple of measures $(\mu_0, \mu_p, \mu)$ satisfying \eqref{eq:liou}
is referred to as a \textbf{relaxed occupation measure}.


% \Iac{ODE} peak estimation problem with adverse time-dependent uncertainty and variables $(t, x_0, u(\cdot))$
% \begin{subequations}
% \label{eq:peak_unc_traj}
%     \begin{align}
%     P^* = & \max_{t^* \in [0, T], \; x_0 \in X_0, \; u(\cdot)} p(x(t^* \mid x_0, u(\cdot))\\
%     & \dot{x} =  f(t, x(t), u(t)), \ u(t) \in U \qquad \forall t \in [0, T]    \\
%     &x(0) = X_0,
%     \end{align}
% \end{subequations}
% has an upper-bounding measure-\ac{LP} with variables $(\mu_0, \mu_p, \mu)$ yielding $p^* \geq P^*$ \cite{miller2021uncertain, lewis1980relaxation}
% \begin{subequations}
% \label{eq:peak_unc_meas}
%     \begin{align}
%         p^* = & \ \sup \quad \inp{p}{\mu_p} \label{eq:peak_meas_obj} \\
%     & \mu_p = \delta_0 \otimes\mu_0 + \pi^{tx}_\# \Lie_f^\dagger \mu \label{eq:peak_meas_flow}\\
%     & \inp{1}{\mu_0} = 1 \label{eq:peak_meas_prob}\\    
%     & \mu_0 \in \Mp{X_0} \label{eq:peak_meas_init} \\
%     & \mu_p \in \Mp{[0, T] \times X} \label{eq:peak_meas_peak} \\
%     & \mu \in \Mp{[0, T] \times X \times U}.\label{eq:peak_meas_occ}    
%     \end{align}
% \end{subequations}
% There is no gap $(P^* = p^*)$ when $[0, T] \times X \times U$ is compact, $p$ is continuous, and $f$ is Lipschitz in $[0, T] \times X \times U$.

 
% A Young Measure \cite{young1942generalized} is a family of probability distributions $\mu_t(u) \in \Mp{U}$ indexed by time. The Young Measure-applied dynamics of \eqref{eq:dynamics_u} is,
% \begin{align}
%     \dot{x}(t) &= \int_U f(t, x(t), u) d \mu_t(u) \label{eq:dynamics_u_young}
% \end{align}

% The conditional Young Measure $\mu_u(u \mid t, x) \in \Mp{U}$ probability distribution may be used to abstract a feedback law. An free-terminal-time averaged occupation measure $\mu$ posed over a stopping time $t^*$, a probability distribution of initial conditions $\mu_0 \in \Mp{X_0}$, and a Young measure $\mu_u(u \mid t, x)$ may be defined with respect to \eqref{eq:dynamics_u_young} and subsets $A \in [0, T], \ B \in X, \ C \in U$,

% \begin{equation}
%     \label{eq:avg_free_occ}
%     \mu(A \times B\times C) = \int_{[0, t^*] \times X_0} I_{A \times B \times C}\left((t, x(t \mid x_0,  u(\cdot)), 
% \end{equation}





% \subsection{Moment-SOS Hierarchy}

==> sections/shaping.tex <==

\subsection{Shaping Constraints}
\label{sec:shaping}
\urg{possibly put this on Arxiv}.
The weak solutions \eqref{eq:weak_multi_fixed} and \eqref{eq:weak_multi_free} assume that the history $x_h(t)$ can vary arbitrarily in time within the support set $H_0$.
% Structure may 
Some applications involve structure in the function class $\mathcal{H}$, such as requiring that the histories in $\mathcal{H}$ are constant in time between $t \in [-\tau_r, 0]$. Examples of these constant histories for the system in \eqref{eq:time_delay_fig} staring within the black box ($H_0$) are plotted in Figure \ref{fig:delay_shape_const}. 

\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{fig/shaping_constant_history.png}
    \caption{Constant histories in the black box}
    \label{fig:delay_shape_const}
\end{figure}


These types of structure in histories may be realized by adding constraints to the weak derivatives of $\mu_h$. One example is enforcing that $x_h(t)$ is constant on $(-\tau_r, 0)$ by,
\begin{align}
    \inp{v(0, x)}{\mu_0} &= \inp{\partial_t v(t, x)}{\textstyle\sum_{i=1}^r\nu_{-i}} +\inp{v(-\tau, x)}{\mu_0}& \forall v \in C([-\tau_r, 0]).
    \label{eq:weak_shaping_open}
\end{align}
A Liouville equation with occupation measure $\mu_h$ may be used to force constant histories on the closed interval $[-\tau_r, 0]$,
\begin{align}
\inp{v(0, x)-v(-\tau_r, x)}{\mu_0}&= \inp{\partial_t v(t, x)}{\textstyle\sum_{i=1}^r\nu_{-i}}  & \forall v \in C([-\tau_r, 0]).
\end{align}

% Content about Lipschitz constraints and continuity, can't figure it out right now.
% Trajectories in $\mathcal{$
% A Lipschitz constraint with Lipschitz constant $L$ in each coordinate $x_k$ 
% and requiring that 
The histories $x_h(t)$ may be filled with lines by setting all second spatial weak derivatives to zero,
\begin{align}
    0 = \inp{\partial_{x_k, x_k'} v(t, x)}{\textstyle\sum_{i=1}^{r} \nu_{-i}}   \qquad \qquad \forall 1 \leq k \leq k' \leq n, \forall v \in C([-\tau_r, 0]).
\end{align}

% Continuity of histories by $-C \leq \partial_t \norm{x_h(t)}_\infty \leq C$ may be realized by the weak derivative shaping constraints,
% \begin{align}
%     -C \leq \inp{\partial_t v(t, x_k)}{\mu_h}   \qquad \qquad \forall  k=1, \ldots,  n, \forall v \in C([-\tau_r, 0] \times ).
% \end{align}


% Lipschitz constraints 



% \subsection{Multiple History Example}



==> sections/summary.tex <==

This paper is organized as follows: Section \ref{sec:preliminaries} formalizes notation and summarizes concepts in measure theory, time-delay, occupation measures, and \ac{ODE} peak estimation. Section \ref{sec:peak_lp} defines an \ac{MV}-solution for free-terminal-time \ac{DDE} solutions to create a measure-\ac{LP} that upper-bounds \eqref{eq:peak_delay_traj}.
Section \ref{sec:moment} reviews the Moment-\ac{SOS} hierarchy and applies it to finding \acp{SDP} to upper-bound the peak-estimation measure \ac{LP}.
Section \ref{sec:examples} provides two examples of \ac{DDE} peak estimation. Section \ref{sec:conclusion} concludes the paper.


==> sections/weak_solutions.tex <==
\section{Weak Solutions of DDEs}

\label{sec:weak_solutions}
\urg{ Revise and Excise this content}

This section develops a measure-valued (weak) solution to a \ac{DDE} of the form in Equation \eqref{eq:delay_dynamics} given a single bounded \ac{PC} history $x_h$. It is further assumed that the terminal time $T$ is finite. 

% \subsection{Motivating Visual Example}
A visual example used throughout this section will be the following trajectory of Equation \eqref{eq:time_delay_fig} with history $x_h(t) = 1 - t/2$ in times $ t \in [-\tau, 0] = [-1, 0]$. This trajectory is plotted in Figure \ref{fig:tri_component} for a time horizon of $T=5$. The blue section between $t \in [-\tau, 0] = [-1, 0]$ is the history $x_h(t)$. The red and green sections of the trajectory are defined in the regions $[0, T-\tau] = [0, 4]$ and $[T-\tau, T] = [4, 5]$ respectively. 

\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{fig/triangle_component_decomposition.pdf}
    \caption{Example trajectory of \eqref{eq:time_delay_fig} to explain \ac{DDE} weak solutions}
    \label{fig:tri_component}
\end{figure}

Figure \ref{fig:tri_stack} shows the trajectory in current time $x(t)$ and in delayed time $x(t-\tau)=x(t-1)$. Note that the data in the red section is identical between current time: $t \in [0, 4]$ and delayed time $t \in [1, 5]$.
\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{fig/triangle_component_stack.pdf}
    \caption{Trajectory in current time and delayed time}
    \label{fig:tri_stack}
\end{figure}

\subsection{Fixed Terminal Time}
\label{sec:weak_fixed}
A weak solution of a controlled time-delay system may be encoded by a tuple of measures $(\mu_T, \bar{\mu}, \{\nu_{j}\}_{j=0}^r)$. The names and supports of these measures are listed in Table \ref{tab:weak_solution}.

\begin{table}[h]
\begin{center}
\caption{\label{tab:weak_solution_old} Description of measures in \ac{DDE} weak solutions}
\begin{tabular}{l l}
    \textbf{Name} & \textbf{Measure and support}  \\
    Terminal & $\mu_T \in \Mp{X_T}$ \\
    Component (start)  & $\nu_0 \in \Mp{[0, T-\tau_r] \times X}$ \\
    Component (end)  & $\nu_{i=1:r} \in \Mp{[T - \tau_{r-i}, T-\tau_{r-i+1}] \times X}$ \\
     Joint Occupation & $\bar{\mu}  \in \Mp{[0, T] \times X^{r+1}}$\\
\end{tabular}
\end{center}
\end{table}
For notational convenience, define the supports of $\nu_j$ as listed in Table 
\ref{tab:weak_solution} as,
\begin{align}
\label{eq:omega_support}
    \Omega_0 &= [0, T-\tau_r] \times X \\
    \Omega_i &= [T - \tau_{r-i}, T-\tau_{r-i+1}] \times X & \forall i= 1, \ldots, r \nonumber.
\end{align}


These measures are related together by a Liouville equation and a set of consistency constraints.

\subsubsection{Liouville Equation}
 
The joint occupation measure $\bar{\mu}(t, x_0, x_1, \ldots, x_r)$ is a Young measure \cite{young1942generalized} 
in terms of time $t$, current state $x_0$, and delayed states $x_i$ for $i=1, \ldots, r$. A joint occupation $\bar{\mu} \in \Mp{[0, T] \times X^{r+1}}$ measure may be formed from every solution $x(t \mid x_h)$ of \eqref{eq:delay_dynamics} satisfying for all test functions $\bar{v} \in C([0, T] \times X^{r+1})$,
\begin{equation}
\label{eq:joint_occ_description}
    \inp{\bar{v}}{\bar{\mu}}=\int_{t=0}^T \bar{v}(t, x(t - \tau_0 \mid x_h), \ldots, x(t - \tau_r \mid x_h)) dt.
\end{equation}

% The correspo
The corresponding terminal measure $\mu_T$ for such a trajectory would be $\mu_T = \delta_{x = x(T \mid x_h)}$.
% A Liouville equation 
The 3-dimensional delay-embedding $(t, x(t), x(t-\tau))$ of the example trajectory is plotted in black in Figure \ref{fig:tri_embedding}. 
% A joint occupation measure $\bar{\mu}$ 
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{fig/triangle_delay_embedding.pdf}
    \caption{Delayed embedding of trajectory in black}
    \label{fig:tri_embedding}
\end{figure}

% A Liou
The Liouville equation in \eqref{eq:liou_meas}-\eqref{eq:liou_int} may be generalized to time-delayed dynamics in \eqref{eq:delay_dynamics}. A Lie derivative for dynamics in \eqref{eq:delay_dynamics} is,
\begin{equation}
    \Lie_f v(t, x_0) = \partial_t v(t,x_0) + f(t, x_0, \ldots, x_r) \cdot \nabla_{x_0} v(t, x_0) \label{eq:delay_lie}
\end{equation}

The time-delay Liouville equation holding for all test functions $v(t, x) \in C^1([0, T] \times X)$ using the Lie derivative in \eqref{eq:delay_lie} is,
\begin{align}
    \inp{v(T, x)}{\mu_T} &= v(0, x_h(0)) + \inp{\Lie_f(t, x_0, \ldots, x_r) v(t, x_0)}{\bar{\mu}} \label{eq:liou_int_delay}\\
    \delta_T \otimes \mu_T &= \delta_0 \otimes \delta_{x=x_h(0)} + \pi^{t x_0}_\# \Lie_f^\dagger \bar{\mu} \label{eq:liou_meas_delay}
\end{align}

% Eq. \eqref{eq:liou_meas_delay} is the Liouville Equation of an 
The Lie derivative $\Lie_f v(t, x)$ in \eqref{eq:liou_int_delay} was expanded to highlight how the delay terms $x(t - \tau_i)$ in dynamics \eqref{eq:delay_dynamics} are replaced by variables $x_i$ in the joint occupation measure $\bar{\mu}$.

\subsubsection{Consistency Constraints}

% Consistency constraints are based on the change-of-variable relation,
% \begin{equation}
%     \int_{0}^T \phi_i(t, x(t - \tau_i)) dt = \int_{-\tau_i}^{T-\tau_i}
%     \end{equation}

The projection of the delay-embedding on the $(t, x(t))$ and $(t, x(t-\tau))$ planes align with the components shown in Figure \ref{fig:tri_stack}. In the measure framework, this projection onto axes corresponds to marginalizations of the joint occupation measures such as $\pi^{t x_i}_\# \bar{\mu}$. Component measures $\{\nu_j\}_{j=0}^r$ are occupation measures in $(t, x)$ containing information about the trajectory in a specific time range, in which the supports are recorded in Table \ref{tab:weak_solution}. As an example with $r=5$ delays, the component measure $\nu_3 \in \Mp{[T-\tau_{2}, T-\tau_{3}]}$ given a trajectory $x(t \mid x_h)$ is the unique occupation measure satisfying $\inp{c_3}{\nu_3} = \int_{T-\tau_3}^{T-\tau_2} \phi_3(t, x(t \mid x_h)) dt$ for all test functions $c_3 \in C([T-\tau_{2}, T-\tau_{3}] \times X)$.

Consistency constraints are imposed between the marginals of $\bar{\mu}$ and time-shifted copies of the component measures $\nu = \{\nu_j\}_{j=0}^r$.  The consistency constraints between $(\bar{\mu}, \nu)$ for lag $i = 0, \ldots, r$ under the convention that $\tau_0 = 0$ may be derived for all $\phi_i \in C([0, T]\times X)$ as,
\begin{align*}
      \inp{\phi_i(t, x_i)}{\bar{\mu}} &= \textstyle\int_{0}^{T} \phi_i(t, x(t  - \tau_i\mid x_h)) dt    & \\
        &= \textstyle\int_{-\tau_i}^{T - \tau_i} \phi_i(t + \tau_i, x(t \mid x_h)) dt  \\
         &= \textstyle\left(\int_{-\tau_i}^{0} + \int_{0}^{T - \tau_i} \right) \phi_i(t + \tau_i, x(t \mid x_h)) dt.
\end{align*}

The final formula for the consistency constraint at lag $i$ is,
\begin{equation}
\label{eq:consistency_single}
    \inp{\phi_i(t, x_i)}{\bar{\mu}} = \textstyle\int_{-\tau_i}^{0} \phi_i(t + \tau_i, x_h(t)) dt + \inp{\phi_i(t + \tau_i, x)}{\textstyle \sum_{j=0}^{r-i} \nu_i}
\end{equation}

% The $x_h$ integration term in \eqref{eq:consistency_single} will evaluate to $0$ by continuity of $\phi_0$ in the current state consistency constraint of $i=0$.


For the trajectory example in Fig \ref{fig:tri_embedding}, the first consistency constraint which holds for all test functions $\phi_0\in C([0, T] \times X)$ is,
    \begin{align*}
        \inp{\phi_0(t, x_0)}{\bar{\mu}} &= \textstyle\int_{0}^{T} \phi_0(t, x(t \mid x_h)) dt   \\
       &= \left(\textstyle\int_{0}^{T-\tau} + \int_{T-\tau}^T \right) \phi_0(t, x(t \mid x_h)) dt \\
       &= \inp{\phi_0(t, x)}{\cz{\nu_0} + \cp{\nu_1}}.
    \end{align*}

The second consistency constraint holding for all test functions $\phi_1\in C([0, T] \times X)$ is,
    \begin{align*}
        \inp{\phi_1(t, x_1)}{\bar{\mu}} &= \textstyle\int_{0}^{T} \phi_1(t, x(t  - \tau\mid x_h)) dt   \\
        &= \textstyle\left(\int_{-\tau}^{0} + \int_{0}^{T - \tau}\right) \phi_1(t + \tau, x(t \mid x_h)) dt  \\
       &=\textstyle \int_{-\tau}^{0} \phi_1(t+\tau, \cn{x_h}(t)) dt  +  \inp{\phi_1(t + \tau, x)}{\cz{\nu_0}}
    \end{align*}

In this manner, the data between times $t \in [0, 4]$ in $\cz{\nu_0}$ is shared between the marginals $\pi_\#^{t x_0} \bar{\mu}$ in current state and $\pi_\#^{t x_1} \bar{\mu}$ in delayed state (visible in Figure \ref{fig:tri_embedding}).

\begin{defn}
A fixed terminal time weak solution of the \ac{DDE} \eqref{eq:delay_dynamics} $(\mu_T, \bar{\mu}, \{\nu_j\}_{j=0}^r)$ given a history $x_h(t): t \in [-\tau_r, 0]$ is a tuple of measures $(\mu_T, \bar{\mu}, \{\nu_j\}_{j=0}^r)$ satisfying the Liouville equation \eqref{eq:liou_meas_delay} and consistency constraints \eqref{eq:consistency_single} for all $i= 0, \ldots, r$.
\end{defn}

\begin{thm}
\label{thm:construct_weak_single_fixed}
Every trajectory $x(t \mid x_h)$ of \eqref{eq:delay_dynamics} has a corresponding weak solution $(\mu_T, \bar{\mu}, \{\nu_j\}_{j=0}^r)$
\end{thm}
\begin{proof}
The proof of the above theorem is interspersed throughout this subsection. The terminal measure may be chosen as $\mu_T = \delta_{x = x(T \mid x_h)}$.  The joint occupation measure is the unique measure obeying Equation \eqref{eq:joint_occ_description}. The zeroth (start) component measure is the unique occupation measure satisfying $\inp{c_0}{\nu_0} = \int_{t=0}^{T-\tau_r} c_0(t, x_h(t)) dt$ for all test functions $c_0\in C([0, T-\tau_r] \times X)$, and the higher (end) component measures $\{\nu_i\}_{i=1}^r$ obey $\inp{c_i}{\nu_i} = \int_{t=T-\tau_{r-i}}^{T-\tau_{r-i+1}} c_i(t, x_h(t)) dt$ for all test functions $c_i\in C([T-\tau_{r-i}, T-\tau_{r-i+1}] \times X)$ and for all $i = 1, \ldots, r$.
\end{proof}

% \begin{thm}
% Every weak solution $(\mu_T, \bar{\mu}, \{\nu_j\}_{j=0}^r)$ given $x_h$ is supported on (portions or embeddings as appropriate of) the trajectory $x(t \mid x_h)$. 
% \label{thm:weak_steps}
% \end{thm}
% \begin{proof}
% The proof of this statement relies on induction through the Method of Steps (Equation \eqref{eq:method_of_steps}). 
% % The joint occupation measure $\bar{\mu}$ may be disentangled into $\bar{\mu}(t, x_0, \ldots, x_r) = \mu_t$

% Define $k_{max} = \ceil{T / \tau_1}$ as the number of steps required to solve a trajectory of \eqref{eq:delay_dynamics}. The joint occupation measure $\bar{\mu}$ may be split into $\bar{\mu} = \sum_{k=1}^{k_{max}} \bar{\mu}^{(k)}$ by absolute continuity where $\bar{\mu}^{(k)} \in \Mp{[(k-1)\tau_1, k \tau_1] \times X^{r+1}}$ for $k < k_{max}$ and $\bar{\mu}^{(k_{max})} \in \Mp{[(k_{max}-1)\tau_1, T] \times X^{r+1}}$.

% Each marginal $\pi^{t x_i}_\# \bar{\mu}^{(1)}$ is supported on the graph $(t, x_h(t - \tau_i))$ between times $[0, \tau_1]$ by consistency constraints \eqref{eq:consistency_single}. Given that the history $x_h: [-\tau, 0] \rightarrow X$ is single-valued for each $t$, the joint marginal $\pi^{t x_1, \ldots x_r} \bar{\mu}^{(k)}$ generated by gluing together the marginals $\pi^{t x_i}_\# \bar{\mu}^{(1)}$ along $t$  is therefore supported on the graph of $(t, x_h(t - \tau_1), \ldots, x_h(t - \tau_r))$.

% The ODE dynamics $F^{(1)}(t, x) = f(t, x, x_h(t - \tau_1), \ldots , x_h(t - \tau_r))$ inspire an ODE Liouville equation \eqref{eq:liou_meas} with initial measure $\mu_0^{(1)} = \delta_{x = x_h(0)}$, terminal measure $\mu_0^{(2)} \in \Mp{X}$, and occupation measure $\mu^{(1)}$,
% \begin{equation}
% \label{eq:step_1_proof}
%     \delta_{t=\tau_1} \otimes \mu_0^{(2)} = \delta_{t=0}\otimes \mu_0^{(1)} + \Lie_{F^{(1)}}^\dagger \mu^{(1)}.
% \end{equation}
% There is a unique solution $(\mu^{(1)}, \mu_0^{(2)})$ to \eqref{eq:step_1_proof} by Theorem 3.1 of \cite{ambrosio2003lecture}.
% Let $x^{(1)}(t)$ be the trajectory starting from $x_h(0)$ obeying
% $\dot{x}^{(1)}(t) = F^{(1)}(t, x)$
% between times $[0, \tau_1]$. 
% The trajectory $x^{(1)}(t)$ is a single-valued function of $t$ for $t \in [0, \tau_1]$.  
% The  measure solution is therefore $\mu_0^{(2)} = \delta_{x = x^{(1)}(\tau_1)}$ and $\mu^{(1)}$ is the occupation measure supported on $(t, x^{(1)}(t))$. 
% The marginal $\pi_\#^{t x_1 \ldots x_0}$ and the occupation measure $\mu^{(1)}$ may be glued together along $t$ to produce the unique occupation measure supported on $(t, x^{(1)}(t), x_h(t - \tau_1), \ldots, x_h(t - \tau_r))$, which is $\bar{\mu}^{(1)}$. 

% Further steps $k=2, \ldots, k_{max}$ may proceed by the same process, patching together a unique weak solution with measures supported on the (portioned and embedded) graphs of the single unique trajectory $x(t \mid x_h)$. For reference, the Liouville equation used in step $k < k_{max}$ is,
% \begin{equation}
% \label{eq:step_k_proof}
%     \delta_{t=k \tau_1} \otimes \mu_0^{(k+1)} = \delta_{t=(k-1) \tau_1}\otimes \mu_0^{(k)} + \Lie_{F^{(k)}}^\dagger \mu^{(k)}.
% \end{equation}


% \end{proof}
% Fo
\subsection{Free Terminal Time}
\label{sec:weak_free}
The weak solutions $(\mu_T, \bar{\mu}, \{\nu_j\}_{j=0}^r)$ described in Section \ref{sec:weak_fixed} have a fixed terminal time $T$. A terminal measure for free terminal time is a probability measure $\mu_p \in \Mp{[0, T] \times X}$, just as in the ODE peak estimation sections. The Liouville equation associated with the free terminal time setting is,
\begin{align}
    \inp{v(t, x)}{\mu_p} &= v(0, x_h(0)) + \inp{\Lie_{f(t, x_0, \ldots, x_r)} v(t, x_0)}{\bar{\mu}} \label{eq:liou_int_delay_free}\\
 \mu_p &= \delta_0 \otimes \delta_{x=x_h(0)} + \pi^{t x_0}_\# \Lie_f^\dagger \bar{\mu}. \label{eq:liou_meas_delay_free}
\end{align}

The consistency constraints in \eqref{eq:consistency_single} must change to accommodate the free terminal time. To explain why, consider the example in Figure \ref{fig:stop_traj}. 

\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{fig/thesis_stop.pdf}
    \caption{Halted execution at $t^*=3$ }
    \label{fig:stop_traj}
\end{figure}

The system \eqref{eq:time_delay_fig} as seen in Figure \ref{fig:tri_stack} is stopped at time $t^* = 3$. The top panel of Figure \ref{fig:stop_traj} shows the trajectory running for $t^*=3$ time units, terminating in the black star. The bottom panel of Figure \ref{fig:stop_traj} is in delayed time units, and the same black star is at time $t^* + \tau = 3+1 = 3$. Let $\bar{\mu}$ be a joint occupation measure obeying consistency constraints \eqref{eq:consistency_single} with respect to $\cz{\nu_0}$ and $\cn{x_h}$. The masses of the marginals (elapsed times) as plotted in Figure \ref{fig:stop_traj} are $\inp{1}{\pi_\#^{t x_0} \bar{\mu}} = 4$ and $\inp{1}{\pi_\#^{t x_1} \bar{\mu}} = 4$. This is a contradiction, since the common $t$-marginals $\pi_\#^t \pi_\#^{t x_0} \bar{\mu}$ and $\pi_\#^t \pi_\#^{t x_1} \bar{\mu}$ should be equal to each other.

This contradiction may be patched by stopping the delayed trajectory $x(t-\tau)$ at time $t^* - \tau$ rather than at time $t^*$. The black star on the bottom panel of Figure \ref{fig:stop_traj_delay} remains at time $t^*+\tau = 4$, but now there is a black circle located at the point $(t^*, x(t^* - \tau\mid x_h)) = (3, x(2))$. This black circle is the stopping point for the delayed process. With the early stop in the black circle, an equal amount of elapsed time occurs in the top plot and the bottom plot. The marginals $t$-marginals $\pi_\#^t \pi_\#^{t x_0} \bar{\mu}$ and $\pi_\#^t \pi_\#^{t x_1} \bar{\mu}$ with delay-stopping are now equal to each other, and a joint occupation measure $\bar{\mu}$ supported on the graph $(t, x(t), x(t - \tau))$ for $t \in [0, t^*]$ may be defined. The dotted red line between the black circle and black star on the bottom plot is the trajectory between times $[t^*-\tau, t^*] = [2, 3]$ in absolute time.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{fig/thesis_stop_free_slack.pdf}
    \caption{Halted execution at $t^*=3$ with delay-stopping}
    \label{fig:stop_traj_delay}
\end{figure}




% \subsection{Single Slacks

The term $\inp{\phi_0(t,x)}{\bar \mu_2}$ may be subtracted from both sides of the zeroth consistency constraint \eqref{eq:consistency_single} at $i=0$, forming the expression,
\begin{equation}
\label{eq:consistency_zero}
    \inp{\phi_0(t,x_0)}{\bar \mu_1} = \inp{\phi_0(t, x)}{\textstyle\sum_{j=0}^r \nu_j} - \inp{\phi_0(t,x_0)}{\bar \mu_2}.
\end{equation}

The supports of the component measures $\{\nu_j\}_{j=0}^r$ form a temporal partition of $[0, T] \times X$. 

By absolute continuity in equation \eqref{eq:consistency_zero}, there exists measures $\nu_j' \in \Mp{\Omega_j}, \ \forall j = 0, \ldots, r$ such that,
\begin{align}
    \inp{\psi_j(t,x)}{\nu_j'} &= \inp{\psi_j(t,x)}{\nu_j} - \int_{\Omega_j} \psi_j(t,x_j)d\bar \mu_2 & \forall \psi_j \in C(\Omega_j). \label{eq:zero_nu_abscont}
\end{align}
The following zeroth consistency constraint no longer involves $\bar{\mu_2}$,
\begin{align}
    \inp{\phi_0(t,x_0)}{\bar \mu_1} &= \inp{\phi_0(t, x)}{\textstyle\sum_{j=0}^r \nu_j'} & \forall \phi_0 \in C([0, T] \times X).
\end{align}

A $\tau_i$-shifted and $[0, T]$-truncated copy of $\pi^{t x_i}_\# \bar{\mu_2}$ (containing trajectory information in times $[t^*+\tau_i, T]$) may now be subtracted from both sides of consistency constraints \eqref{eq:consistency_single} for all $i = 1, \ldots, r$,
\begin{subequations}
\label{eq:consistency_shift}
\begin{align}
    \Phi_i &= \textstyle\inp{\phi_i(t, x_i)}{\bar{\mu_1} + \bar{\mu}_2} - \int_{[0, T-\tau_i] \times X} \phi_i(t + \tau_i, x_0) d \bar{\mu} \label{eq:consistency_shift_lhs}\\
    &= \textstyle\int_{t=-\tau_i}^0 \phi_i(t+\tau_i, x_h(t)) dt + \inp{\phi_i(t+\tau_i, x)}{ \sum_{j=0}^{r-i} \nu_i} - \int_{[0, T-\tau_i] \times X} \phi_i(t + \tau_i, x_0) d \bar{\mu}_2. \label{eq:consistency_shift_rhs}
\end{align}
\end{subequations}
The bottom term \eqref{eq:consistency_shift_rhs} may be reformulated using the $\{\nu_j\}_{j=0}^r$ expressions from \eqref{eq:zero_nu_abscont},
\begin{equation}
    \Phi_i = \textstyle\int_{t=-\tau_i}^0 \phi_i(t+\tau_i, x_h(t)) dt + \inp{\phi_i(t+\tau_i, x)}{ \sum_{j=0}^{r-i} \nu_i'}.
\end{equation}

The top term may also be reformulated via absolute continuity. There exists a nonnegative measure $\hat{\nu}_i \in \Mp{[0, T] \times X}$ such that,
\begin{equation}
    \inp{\phi_i(t, x_i)}{\bar{\mu_2}} = \inp{\phi_i(t, x)}{\hat{\nu}_i} +\int_{[0, T-\tau_i] \times X} \phi_i(t + \tau_i, x_0) d \bar{\mu}_2.
    \label{eq:i_nu_abscont}
\end{equation}

Let $t^*$ be a stopping time in the support of $\pi^t_\# \mu_p$. The measure $\pi^{t x_i}_\# \bar{\mu_2}$ in the left hand side of \eqref{eq:i_nu_abscont} is supported in times $[t^*, T]$. The $\tau_i$-shifted and truncated copy of $\pi^{t x_0}_\# \bar{\mu_2}$ (rightmost integral term of \eqref{eq:i_nu_abscont}) is supported in time $[t^*+\tau_i, T]$. The remaining slack term $\hat{\nu}_i$ is therefore supported on the trajectory in times $[t^*, t^*+\tau_i]$. This support is illustrated by the red dotted line after the black circle in the bottom plot of Figure \ref{fig:stop_traj_delay}. The red curve on the top plot of Figure \ref{fig:stop_traj_delay} is the support of $\cz{\nu_0'}$ in [0, 4], and $\cp{\nu_1'}$ in this example is the zero measure.

An expression for the free-time consistency constraint \eqref{eq:consistency_shift} for all $i = 1, \ldots, r$ and $\phi_i \in C([0, T] \times X)$ is,
\begin{equation}
\label{eq:consistency_slack}
    \Phi_i = \inp{\phi_i(t, x)}{\bar{\mu}_1}+ \inp{\phi_i(t, x)}{\hat{\nu}_i} = \textstyle\int_{t=-\tau_i}^0 \phi_i(t+\tau_i, x_h(t)) dt + \inp{\phi_i(t+\tau_i, x)}{ \sum_{j=0}^{r-i} \nu_i'}.
\end{equation}

There is a single slack measure $\hat{\nu}_i$ in each consistency constraint \eqref{eq:consistency_slack} for $i=1, \ldots, r$. 
% The joint occupation measure $\bar{\mu}_2$ over arbitrary dynamics has been completely eliminated from the consistency constraint expression.

\begin{defn}
A tuple $(\mu_p, \ \bar{\mu}, \  \{\nu_j\}_{j=0}^r, \ \{\hat{\nu}_i\}_{i=1}^r)$ is a free-time weak solution to a system with dynamics \eqref{eq:delay_dynamics} and a given history $x_h$ if it satisfies constraints,
\begin{subequations}
\begin{align}
&\forall v \in C^1([0, T] \times X):  \\
    & \qquad \inp{v(t,x)}{\mu_p} = v(0, x_h(0)) + \inp{\Lie_f v(t, x)}{ \bar{\mu}}  \nonumber  \\
    & \forall \phi_0 \in C([0, T] \times X):   \\
    & \qquad \inp{\phi_0(t, x_0)}{\bar{\mu}} = \inp{\phi_0(t, x)}{ \textstyle \sum_{j=0}^{r} \nu_i}\nonumber \\
    & \forall \phi_i \in C([0, T] \times X), \forall i=1, \ldots, r: \\
    &\qquad \inp{\phi_i(t, x)}{\bar{\mu}}+ \inp{\phi_i(t, x)}{\hat{\nu}_i} = \textstyle\int_{t=-\tau_i}^0 \phi_i(t+\tau_i, x_h(t)) dt + \inp{\phi_i(t+\tau_i, x)}{ \sum_{j=0}^{r-i} \nu_i} \nonumber \\
    &\mu_p \in \Mp{[0, T] \times X}, \ \bar{\mu} \in \Mp{[0, T] \times X^{r+1}}, \  \nu_0 \in \Mp{[0, T- \tau_r] \times X} \\
    & \forall i = 1, \ldots, r: \nu_i \in \Mp{[T - \tau_{r-i}, T - \tau_{r-i+1}] \times X}, \ \hat{\nu}_i \in \Mp{[0, T] \times X}.
\end{align}
\end{subequations}
\end{defn}

\begin{thm}
\label{thm:delay_single_free}
A free-time weak solution may be constructed from every trajectory $x(t\mid x_h)$ starting from $x_h$ stopping at time $t^* \in [0, T]$.
\end{thm}
\begin{proof}
% The content of this proof is dispersed in prior sections. 
The terminal measure may be chosen to be $\mu_p = \delta_{t = t^*} \otimes \delta_{x = x(t^* \mid x_h)}$. The component measures satisfy $\inp{\phi_0(t, x)}{\sum_{j=0}^r \nu_j} \ \int_{t=0}^{t^*} \phi_0(t, x(t \mid x_h)) dt$ for all $\phi_0 \in C([0, T] \times X)$. The joint occupation measure $\bar{\mu}$ is the occupation measure supported on the graph of $(t, x(t \mid x_h), x(t - \tau_1 \mid x_h), \ldots, x(t - \tau_r \mid x_h))$ in times $t \in [0, t^*]$. For each $i = 1, \ldots, r$, the slack measure $\hat{\nu}_i$ is the unique occupation measure satisfying $\inp{\phi_i(t, x)}{\hat{\nu}_i} =  \ \int_{t=t^*}^{\min(T, t^* + \tau_i)} \phi_i(t, x(t - \tau_i \mid x_h)) dt$.
\end{proof}  

% \begin{thm}
% \label{thm:delay_single_free_parameterized}
% Every free-time weak solution is supported on a family of trajectories parameterized by the stopping time $t^*$ of \eqref{eq:delay_dynamics} starting from $x_h$.
% \end{thm}
% \begin{proof}
% % The proof of this theorem relies on undoing the work in this subsection to recover a Two-Liouville expression. A measure $\bar{\mu_2} \in $

% This theorem may be proved by varying the Method of Steps construction used in the proof of Theorem \ref{thm:weak_steps}. 
% The terminal measure $\mu_p \in \Mp{[0, T] \times X}$ may be split into the sum of measures $\mu_p^{(k)} \in \Mp{[(k-1)\tau_1, k \tau_1]}$ and $\mu_p^{(k_{max})} \in \Mp{[(k_{max}-1)\tau_1, T] \times X}$ by absolute continuity.
% The step between times $t \in [0, \tau_1]$ obeys ODE dynamics  $\dot{x}(t) = F^{(1)}(t, x) = f(t, x, x_h(t - \tau_1), \ldots , x_h(t - \tau_r))$. An ODE Liouville equation \eqref{eq:liou_meas} with initial measure $\mu_0^{(1)} = \delta_{x = x_h(0)}$, terminal measure $\mu_0^{(2)} \in \Mp{X}$, mid-time terminal measure $\mu_p^{(1)} \in \Mp{[0, \tau_1] \times X}$ from $\mu_p$ (split by absolute continuity), and occupation measure $\mu^{(1)} \in \Mp{[0, \tau] \times X}$,
% \begin{equation}
% \label{eq:step_1_proof_free}
%     \delta_{t=\tau_1} \otimes \mu_0^{(2)} + \mu_p^{(1)} = \delta_{t=0}\otimes \mu_0^{(1)} + \Lie_{F^{(1)}}^\dagger \mu^{(1)}.
% \end{equation}

% The free-terminal measure $\mu_p^{(1)}$ captures the distribution (endpoints) of trajectories that stop in times $t \in [0, T]$. Delayed versions of these terminated trajectories are recorded until times $t^* + \tau_i$ (where $t^*$ is distributed as $\pi_\#^t \mu_p^{(1)}$) by the slacks $\hat{\nu}_i$, as enforced by the consistency constraint \eqref{eq:consistency_slack}. The Liouville equation at step $k < k_{max}$ is,
% \begin{equation}
% \label{eq:step_k_proof_free}
%     \delta_{t=k\tau_1} \otimes \mu_0^{(2)} + \mu_p^{(k)} = \delta_{t=(k-1) \tau_1}\otimes \mu_0^{(k)} + \Lie_{F^{(k)}}^\dagger \mu^{(k)},
% \end{equation}
% and the Liouville equation at step $k_{max}$ is,
% \begin{equation}
% \label{eq:step_k_proof_free_liou}
%     \mu_p^{(k_{max})} = \delta_{t=(k_{max}-1) \tau_1}\otimes \mu_0^{(k_{max})} + \Lie_{F^{(k_{max})}}^\dagger \mu^{(k_{max})}.
% \end{equation}
% By ODE uniqueness arguments from Theorem 3.1 of \cite{ambrosio2003lecture} in each step, the single-slack free-time weak solution is supported on a family of trajectories starting from $x_h$. The parameterizing stopping times $t^*$ are distributed as the $t$-marginal $\pi^t_\# \mu_p$. 

% \end{proof}
% As described in the previous derivations, every free-time stopped trajectory may be represented as a weak solution, and every weak solution is supported on a family of trajectories starting from $x_h$.
\section{Weak Solutions with Multiple Histories}

\label{sec:weak_multiple}

The weak solutions that have previously been developed in this section were defined with a single given history $x_h(t): \ t \in [-\tau_r, 0]$. This section will develop weak solutions where the initial histories $x_h$ are members of a function class $\mathcal{H} \subset PC([-\tau, 0] \times X)$. An example could be where $\mathcal{H}$ is the set of histories defined between times $t \in [-2, 0]$ with $1 \leq x_h(t) \leq 2$ and containing no further constraints on continuity of histories.
% are drawn from a distribution of histories (occupation measures between times $t \in [-\tau_r, 0]$).

Let the set $H_0 \subset [-\tau_r, 0] \times X$
contain the graph of all admissible initial state histories,
\begin{equation}
    (t, x_h(t)) \in H_0 \qquad \forall t \in [-\tau_r, 0], \qquad \forall x_h \in \mathcal{H}.
\end{equation}
Further define the set $X_0$ of initial conditions at time $t=0$ as the slice,
\begin{equation}
    X_0 = \{x \mid (0^+, x) \in H_0\}.
\end{equation}

\subsection{Fixed Terminal Time}
In this weak solution framework, the admissible trajectories $x_h(t) \in \mathcal{H}$ are distributed (averaged)
% The histories $x_h(t)$ are distributed  
according to an occupation measure $\mu_h \in \Mp{H_0}$. In the case of a single history $x_h$, this history occupation measure is the unique measure satisfying $\inp{v(t, x)}{\mu_h} = \int_{-\tau_r}^0 v(t, x_h(t)) dt$.

Define the support sets $\{\Omega_{-i}\}_{i=1}^r$ and history components $\{\nu_{-i}\}_{i=1}^r$,
\begin{align}
    \Omega_{-i} &= ([-\tau_i, -\tau_{i-1}] \times X) \cap H_0  & & i = 1, \ldots, r \\
    \nu_{-i} &\in \Mp{\Omega_{-i}}.
\end{align}
The support sets $\Omega_{-i}$ complement the existing $\Omega_{\geq 0}$ definition in Equation \eqref{eq:omega_support}.
The history occupation measure $\mu_h$ may be split by absolute continuity into the sum of history component measures $\mu_h = \sum_{i=1}^r \nu_{-i}$.

Consistency constraints with history occupation measures and fixed terminal time are,
\begin{align}
\label{eq:consistency_multi_fixed}
    \inp{\phi_i(t, x_i)}{ \bar{\mu}} &= \inp{\phi_i(t, x)}{\textstyle\sum_{j=-i}^{r-i} \nu_j} & \forall \phi_i \in C([0, T] \times X), i=0, \ldots, r.
\end{align}

An equivalent expression for constraint \eqref{eq:consistency_multi_fixed} is,
\begin{align}
\pi^{t x_i}_\# \bar{\mu} &= \textstyle \sum_{j=-i}^{r-i} \nu_j & \forall i = 0, \ldots, r.
\end{align}

The following definition will assume that the class $\mathcal{H}$ is the set of bounded \ac{PC} histories whose graph is inside $H_0$ with no further constraints.
\begin{defn}
\label{defn:weak_multiple_fixed}
A fixed terminal time weak solution with histories in $H_0$ is a tuple $(\mu_0, \mu_T, \bar{\mu}, \{\nu_j\}_{j=-r}^r)$ subject to,
\begin{subequations}
\label{eq:weak_multi_fixed}
\begin{align}
    &\inp{v(T, x)}{\mu_T} = \inp{v(0, x)}{\mu_0} + \inp{\Lie_f v(t, x)}{\bar{\mu}} & &\forall v \in C^1([0, T] \times X)  \\
    &\inp{\phi_i(t, x_i)}{\bar{\mu}} = \inp{\phi_i(t+\tau_i, x)}{\textstyle \sum_{j=-i}^{r-i} \nu_j} & &\forall \phi_i \in C([0, T] \times X), \ i = 0, \ldots, r \\
    & \inp{1}{\mu_0} = 1 \\
    &\mu_0 \in \Mp{X_0}, \ \mu_{T} \in \Mp{X} \\
    &\bar{\mu} \in \Mp{[0, T] \times X^{r+1}} \\
    &\nu_j \in \Mp{\Omega_j} & &\forall j = -r, \ldots, r.
\end{align}
\end{subequations}
\end{defn}

\begin{thm}
\label{thm:delay_multiple_fixed}
A multiple-history weak solution may be constructed from every trajectory $x_h(t) \in \mathcal{H}$ (satisfying $(t, x_h(t)) \in H_0 \  \forall t \in [-\tau_r, 0]$).
\end{thm}
\begin{proof}
This construction follows the method in Theorem \ref{thm:construct_weak_single_fixed} to form the measures $\mu_T, \bar{\mu}, \{\nu_j\}_{j=0}^r$ from the given history $x_h$. The initial measure may be chosen $\mu_0 = \delta_{x=x_h(0)}$, and the history components respect $\inp{v(t, x)}{\nu_{-i}} = \int_{-\tau_{i}}^{-\tau_{i-1}} v(t, x_h(t)) dt$ for all $v \in C([-\tau_i, -\tau_{i-1}] \times X)$ and $i = 1, \ldots, r$.
Conic combinations of weak solutions formed by histories $x_h^1, x_h^2, \ldots \in \mathcal{H}$ will also be a multiple-history weak solution by convexity of constraints in \eqref{eq:weak_multi_fixed}.
\end{proof}


% Free terminal time consistency constraints with multiple occupation measures have a term $\inp{\phi_i(t, x_i)}{ \bar{\mu} + \nu_i}$ on the left hand side of \eqref{eq:consistency_multi_fixed}, just as in Equation \eqref{eq:consistency_slack}.

% Future work includes finding out under what conditions will multiple-history weak solutions \eqref{eq:weak_multi_fixed}  be supported along \ac{DDE} trajectories of \eqref{eq:delay_dynamics}. A first step from \cite{lewis1980relaxation} may be that the image of the map $X^r \rightarrow f(t, x_0, X, X, X, \ldots, X)$ is convex for each fixed $(t, x_0) \in [0, T] \times X$. 
% If this convexity condition holds, $[0, T] \times X$ is compact, and $f$ is Lipschitz, then weak solutions \eqref{eq:weak_multi_fixed} are supported on the graphs of trajectories $x_0' = f(t, x_0, x_1, x_2, \ldots x_r)$ with external inputs $x_1(t), \ldots x_r(t)$ \cite{korda2014convex}. It is unknown at this point whether the consistency constraints \eqref{eq:consistency_multi_fixed} are strong enough to force the external inputs to align with delayed trajectories as $x_i(t) = x_0(t - \tau_i)$.

\subsection{ Free Terminal Time}

Free terminal time weak solutions with multiple histories require a set of additional constraints in order for all measures to remain bounded when $\mu_h$ is not given a priori. To explain why, consider free-time consistency constraint with multiple histories at delay $i = 1, \ldots, r$,
\begin{align}
\label{eq:consistency_multi_free}
    \inp{\phi_i(t, x_i)}{\bar{\mu}} + \inp{\phi_i(t, x)}{\nu_i} &= \inp{\textstyle \phi_i(t+\tau_i, x)}{ \sum_{j=-i}^{r-i} \nu_j} & \forall \phi_i \in C([0, T] \times X).
\end{align}

The case with $r=1$ will lead to the following expressions,
\begin{subequations}
\label{eq:free_time_example}
\begin{align}
\text{Initial Prob. Measure:} & & \inp{1}{\mu_0} &= 1 \label{eq:free_time_example_prob}\\
\text{Liouville $v(t, x)=1$:} & & \inp{1}{\mu_p} &= \inp{\partial_t 1}{\bar{\mu}} + \inp{1}{\mu_0} =  \inp{1}{\mu_0} = 1 \\
    \text{Liouville $v(t, x)=t$:} & & \inp{t}{\mu_p} &= 0 *\inp{1}{\mu_0}+\inp{\partial_t t}{\bar{\mu}} =  \inp{1}{\bar{\mu}} \leq T \\
    \text{Consistency $\phi_0(t, x)=1$:} & & \inp{1}{\bar{\mu}} &= \inp{1}{\nu_0 + \nu_1} \label{eq:free_time_example_consistency}\\
    \text{Consistency $\phi_1(t, x)=1$:} & & \inp{1}{\bar{\mu}} &= \inp{1}{\nu_0} + (\inp{1}{\nu_{-1}} - \inp{1}{\hat{\nu}_1}) \label{eq:free_time_example_error}.
\end{align}
\end{subequations}
The masses of $\mu_0, \mu_p, \bar{\mu}, \nu_0, \nu_1$ are all bounded by constraints \eqref{eq:free_time_example_prob}-\eqref{eq:free_time_example_consistency} when $T$ is finite. Line \eqref{eq:free_time_example_error} enforces a mass constraint involving the difference
$\inp{1}{\nu_{-1}} - \inp{1}{\hat{\nu}_1}$.
The mass $\inp{1}{\hat{\nu}_1}$ is only present and constrained  in this free-time consistency expression, so therefore the masses of $\nu_{-1}$ and $\hat{\nu}_1$ may each be unbounded. 

More generally, the masses of $\{\nu_{-i}, \hat{\nu}_i\}_{i=1}^r$ may be unbounded in a na\"ive porting of the multiple-history weak solution \eqref{eq:weak_multi_fixed} to free terminal time.

This issue of unbounded masses may be fixed by adding a Lebesgue constraint to the time marginals of the history components. The history occupation measure $\mu_h = \sum_{i=1}^r \nu_{-i}$ should represent a distribution of histories $x_h \in PC(H_0)$, where each history $x_h(t)$ is defined in times $t \in [-\tau_r, 0]$. The $t$-marginal $\pi^t_\# \mu_h$ should therefore be equal to the Lebesgue measure $\lambda_{[-\tau_r, 0]}$,
% \begin{align}
%     \inp{w(t)}{\sum_{i=1}^r \nu_{-i}} &= \int_{t = -\tau_r}^0 w(t) dt & \forall w \in C([-\tau_r, 0]).
% \end{align}
As a consequence, the mass $\inp{1}{\mu_h} = \tau_r$ under this Lebesgue constraint would equal the elapsed time in histories between $[-\tau_r, 0]$. The history components have mass $\nu_{-i} = \tau_i - \tau_{i-1} \ \forall i = 1, \ldots, r$.

\begin{defn}
\label{defn:weak_multiple_free}
A free terminal time weak solution with histories supported in $H_0$ is a tuple $(\mu_0, \mu_T, \bar{\mu}, \{\nu_j\}_{j=-r}^r, \{\hat{\nu_i}\}_{i=1}^r)$ subject to,
\begin{subequations}
\label{eq:weak_multi_free}
\begin{align}
    &\inp{v(T, x)}{\mu_T} = \inp{v(0, x)}{\mu_0} + \inp{\Lie_f v(t, x)}{\bar{\mu}} & &\forall v \in C^1([0, T] \times X)  \\
    &\inp{\phi_i(t, x)}{\hat{\nu}_i \pi^{t x_i}_\#\bar{\mu}} = \inp{\phi_i(t+\tau_i, x)}{\textstyle \sum_{j=-i}^{r-i} \nu_j} & &\forall \phi_i \in C([0, T] \times X), \ i = 0, \ldots, r \\
    & \inp{1}{\mu_0} = 1 \\
    &\inp{h(t)}{\textstyle\sum_{i=1}^r \nu_{-i}} = \textstyle\int_{t = -\tau_r}^0 h(t) dt & & \forall h \in C([-\tau_r, 0]). \\
    &\mu_0 \in \Mp{X_0}, \ \mu_{T} \in \Mp{X} \\
    &\bar{\mu} \in \Mp{[0, T] \times X^{r+1}} \\
    &\nu_j \in \Mp{\Omega_j} & &\forall j = -r, \ldots, r.
\end{align}
\end{subequations}
\end{defn}

\begin{thm}
\label{thm:delay_multiple_free}
A multiple-history free-time weak solution stopping at time $t^*$ may be built from every trajectory $x_h(t) \in \mathcal{H}$.
\end{thm}
\begin{proof}
The measures $\mu_T, \bar{\mu}, \{\nu_j\}_{j=0}^r, \{\hat{\nu_i}\}_{i=1}^r$ may be formed per the proof of Theorem \ref{thm:delay_single_free}. The measures $\{\hat{\nu_{-i}}\}_{i=1}^r$ and $\mu_0$ may be created based on the proof of Theorem \ref{thm:delay_multiple_fixed}. The measure $\mu_h = \sum_{i=1}^r \nu_{-i}$ is the unique occupation measure representing the history $x_h(t): t \in [-\tau_r, 0]$, so it automatically satisfies the time-Lebesgue constraint $\pi^t_\# \mu_h = \lambda_{[-\tau_r, 0]}$.
\end{proof}

It is as of yet unknown whether the converse of Theorem \ref{thm:delay_multiple_free} holds, whether every multiple-history free-time weak solution is supported on a family of \ac{DDE} trajectories. An  answer of validity to the converse of Theorem \ref{thm:delay_multiple_fixed} on fixed terminal time is required before working on the free terminal time case.

% \urg{Try out multiple histories on the SIR demo with constant histories. Randomly sample constant histories $x_h(t) = (1-I_0, I_0)$ as $I_0$ is drawn from a uniform distribution. Compute expected moments of the occupatoin measure by simulation as well as through the LMI.}


==> sections_arxiv/contributions_arxiv.tex <==

The contributions of this paper are:
\begin{itemize}
    \item A theory of \ac{MV}-solutions to \acp{DDE} with multiple histories (in $\hs$) and free terminal time
    \item A measure \ac{LP} that upper-bounds problem \eqref{eq:peak_delay_traj}
    \item A convergent sequence of \acp{LMI} (and resultant \acp{SDP}) to the measure upper-bound
    \item A proof of strong duality for the measure \ac{LP}
\end{itemize}
